New developments in the theory of Groebner bases and applications to formal verification

We present foundational work on standard bases over rings and on Boolean Groebner bases in the framework of Boolean functions. The research was motivated by our collaboration with electrical engineers and computer scientists on problems arising from formal verification of digital circuits. In fact, algebraic modelling of formal verification problems is developed on the word-level as well as on the bit-level. The word-level model leads to Groebner basis in the polynomial ring over Z/2n while the bit-level model leads to Boolean Groebner bases. In addition to the theoretical foundations of both approaches, the algorithms have been implemented. Using these implementations we show that special data structures and the exploitation of symmetries make Groebner bases competitive to state-of-the-art tools from formal verification but having the advantage of being systematic and more flexible.

==> about_pbori.tex <==
\section{The \PolyBoRi Framework}

With \PolyBoRi, we have implemented a C++ library for \emph{Poly}nomials over
\emph{Bo}olean \emph{Ri}ngs, which provides high-level
data types for Boolean polynomials and monomials, exponent vectors, as well as
for the underlying polynomial rings.
The ring variables may be identified by their indices or by a custom string.
%
Polynomial structures and monomials use ZDDs as internal storage type, but this
is hidden from the user.  The current implementation uses the decision-diagram
management from CUDD~\citep{somenzi05cudd}. Its functionality is included using interface
classes, which allows an easy replacement of the underlying BDD system without
extensive rewriting of crucial \PolyBoRi procedures.

In addition, basic polynomial operations~-- like addition and multiplication~--
have been implemented and associated to the corresponding operators. 
In order to enable efficient implementation, 
these operations were reformulated in terms of set operations, which are
compatible with the ZDD approach.
This also applies to other classical functionality like degree computation and
leading-term computations. The ordering-dependent functions are currently
available for lexicographical, degree-lexicographical~(graded-lexicographical) ordering (with first
variable being the largest one),
and degree-reverse-lexicographical ordering, whereas in the latter case
the variables are treated in reversed order for efficiency reasons.
Product orderings consisting of blocks of these are also available.

A complete Python \citep{RossumPython01} interface allows for parsing of complex polynomial systems, 
and also sophisticated and easy extendable strategies for \Groebner base
computations have been made possible by this.
%
An extensive testsuite, which
mainly carries satisfiability examples, and also some from cryptography,
is used to ensure validity during development.
Also, with the tool ipython the \PolyBoRi data structures and procedures can
be used interactively as a command line tool.
In addition, routines for interfacing with the computer algebra system \Singular{}~\citep{GPS05} are under development.

\subsection{Polynomial Arithmetic}
\label{sec:poly_arith}
Boolean polynomial rings are motivated by the fact, that logical
operations on bits can be reformulated in terms of addition and multiplication
of~$\mathbb{Z}_2$-valued variables. 
%
Representing polynomials as ZDDs these operations may also be implemented as set
operations.
\ifx\itwmrep\undefined{For instance, }\else{E.\,g., }\fi 
adding the 
polynomials~$p =  \sum_{s\in S_p} \left( \prod_{x_\nu \in s}x_\nu \right)$
and~$q =  \sum_{s\in S_q} \left( \prod_{x_\nu \in s}x_\nu \right)$,
with~$S_p$ and~$S_q$ as illustrated in \eqnref{eqn:rewrittenpoly}~(% 
\secref{sec:rewrittenpoly}), is just
$p + q =  \sum_{s\in S_{p+q}} \left( \prod_{x_\nu \in s}x_\nu \right)$,
where~$S_{p+q} = (S_p\cup S_q) \backslash  (S_p\cap S_q)$.
Although each of these three operations is already available for ZDDs, it is
usually more preferable to have them replaced by one \specialised procedure. This
avoids large intermediate sets (like~$S_p\cup S_q$) and repeated iterations over
both arguments. 

\Algref{alg:recursive_add} shows a suitable implementation of the Boolean
polynomial addition.
%
\begin{algorithm}[htb]
\caption{Recursive Boolean addition }
\label{alg:recursive_add}
\begin{algorithmic}
\REQUIRE $f, g$ Boolean Polynomials
\ENSURE $h = f+g$
\IF{$f = 0$}
\STATE  $h = g$
\ELSIF{$g = 0$}
\STATE  $h = f$
\ELSIF{$f = g$}
\STATE  $h = 0$
\ELSE
\IF{$\mathrm{isCached}(+, f, g)$}
\STATE $h =\mathrm{cache}(+, f, g)$
\ELSE

\STATE set $x_\nu = \mathrm{top}(f)$,  $x_\mu = \mathrm{top}(g)$

\IF{$\nu < \mu$}
\STATE $h = \ite(x_\nu, \thenBranch(f),  \elseBranch(f) + g) $
\ELSIF{$\nu > \mu$}
\STATE $h = \ite(x_\mu, \thenBranch(g), f + \elseBranch(g)) $
\ELSE
\STATE $h = \ite(x_\nu, \thenBranch(f) + \thenBranch(g),
                                \elseBranch(f) + \elseBranch(g) ) $
\ENDIF
\STATE $\mathrm{cache}(+, f, g) = h$
\ENDIF
\ENDIF
\RETURN $h$
\end{algorithmic}
\end{algorithm}
%
%Note that~$\mathrm{top}(p) = \min \bigcup_{s\in S_p}{s}$ denotes the variable
%associated to the root node of the current ZDD. 
%Also, then- or else-branch of the latter correspond to polynomials referred to
%as~$\mathrm{then}(p)$ and~$\elseBranch(p)$, respectively.
Since the indices of~$\mathrm{top}(p), \mathrm{top}(q)$ are greater than~$i$,
the {if-then-else operator} $\mathrm{ite}(x_i, p, q)$, which 
is equivalent to~$ x_i\cdot p +q$  here,
can be implemented cheaply  by linking then- and else-branches of the new root node
for~$x_i$ to~$p$ and~$q$, respectively.

The procedure also includes a cache lookup, immediately after the initial
if-statements, which treat trivial cases only.
%
The lookup can be implemented cheaply, because polynomials 
have a unique representations as ZDDs.
%
Hence, previous computations  of the sums of the form~$f+g$ can be reused.
The advantage of a recursive formulation is, that
this also applies to those subpolynomials, which are
generated by~$\thenBranch(f)$ and~$\elseBranch(f)$.
%
Because of the recurring
multiplication and addition operations, which are used
in Buchberger-based algorithms for elimination of leading terms and the
tail-reduction process,
it is very likely, that common subexpressions can be reused during
\Groebner base computation.
%
Currently, the default settings of the underlying BDD
library are used for cache-size and related parameters.
Fine-tuning and \optimisation in this area are subject of further research.


In a similar manner a kind of Boolean multiplication is given in
\algref{alg:recursive_mult}.
%
\begin{algorithm}[htb]
\caption{Recursive Boolean multiplication}
\label{alg:recursive_mult}
\begin{algorithmic}
\REQUIRE $f, g$ Boolean Polynomials
\ENSURE $h = f\boolemult g$
\IF{$f = 1$}
\STATE  $h = g$
\ELSIF{$f = 0$ or $g = 0$}
\STATE  $h = 0$
\ELSIF{$g = 1$ or $f = g$}
\STATE  $h = f$
\ELSE
\IF{$\mathrm{isCached}(\boolemult, f, g)$}
\STATE $h =\mathrm{cache}(\boolemult, f, g)$
\ELSE
\STATE  $x_\nu = \mathrm{top}(f)$,  $x_\mu = \mathrm{top}(g)$

\IF{$\nu < \mu$}
\STATE set $p_1 =\thenBranch(f)$, $p_0 =\elseBranch(f)$,
$q_1 = g$, $q_0 = 0$
\ELSIF{$\nu > \mu$}
\STATE set $p_1 =\thenBranch(g)$, $p_0 =\elseBranch(g)$,
$q_1 = f$, $q_0 = 0$
\ELSE
\STATE set $p_1 =\thenBranch(f)$, $p_0 =\elseBranch(f)$,
$q_1 =\thenBranch(g)$, $q_0 =\elseBranch(g)$
\ENDIF
\STATE $h = \ite(x_{\min(\nu, \mu)}, p_0\boolemult q_1 + p_1\boolemult q_1 + p_1 \boolemult q_0,  p_0
\boolemult q_0 ) $
\STATE $\mathrm{cache}(\boolemult, f, g) = h$
\ENDIF
\ENDIF
\RETURN $h$
\end{algorithmic}
\end{algorithm}
%
The procedure computes the unique
representative of the product of two Boolean polynomials modulo the field
equations. This 
multiplication is denoted by~\boolemult\ in the following, while~$\cdot$ means
the usual multiplication. If variables of right- and left-hand side polynomials
are distinct, both operations coincide.

\subsection{Monomial Orderings}
The operations treated in \secref{sec:poly_arith} are independent of the actual
monomial ordering. Crucial for \Groebner algorithms is the computation of the
\defemph{leading term} or \defemph{leading monomial}. Both concepts are equal in
our context, and mean the largest monomial, with respect to the
current~``$<$''-relation. 

It was a major part of our research to make
such functionality available for various nontrivial monomial orderings.
In particular, this applies to such orderings, which obviously do not match 
with the natural order of the terms stored by a ZDD.
%
By taking advantage of the cache and the  uniqueness properties of the data
structure is was possible to implement  these functions
with a reasonable small computational overhead.

Lexicographically, the \defemph{leading monomial} is
just the product of all node variables in the first valid path of the underlying
ZDD, \ie the sequence of nodes from the root down
to the~1-leaf consisting of those
nodes adjacent by then-branches only.
%
In case of degree orderings, one has to work harder.
For instance, the leading monomial for the degree-lexicographical ordering can
be found by iterating over all monomials~(see \secref{sec:iterators}) as
follows: initially, degree and monomial of the first term are stored. If
incrementing to the next term leads to a strictly higher degree, both~-- degree and
monomial~-- are replaced by the current ones. This na{\"i}ve approach does not
make use of recursions, and hence it cannot be cached efficiently. 
A more suitable variant is given in \algref{alg:recursive_lead_deg_dlex}. 

\begin{algorithm}
\caption{Recursive leading term and degree  
$\mathrm{lead\_and\_deg}(f)$  (degree-lex.)}
\label{alg:recursive_lead_deg_dlex}
\begin{algorithmic}
\REQUIRE $f$ Boolean polynomial.
\ENSURE $ \{h, d\} = \{\mathrm{lead}(f), \deg(f)\}$
\IF{$f$ is constant}
\STATE  $h = 1$, $d = 0$ 
\ELSE
\IF{$\mathrm{isCached}(\mathrm{lead\_and\_deg}, f)$}
\STATE $\{h, d\} = \mathrm{cache}(\mathrm{lead\_and\_deg}, f)$
\ELSE
\STATE  $\{h_1, d_1\} = \mathrm{lead\_and\_deg}(\thenBranch(f))$
\STATE  $\{h_0, d_0\} = \mathrm{lead\_and\_deg}(\elseBranch(f))$
\IF{$d_0 < d_1 + 1$}
\STATE $h = \mathrm{top}(f)\cdot h_1$, $d = d_1+1$
\ELSE
\STATE $h = h_0$, $d = d_0$
\ENDIF
\STATE  $\mathrm{cache}(\mathrm{lead\_and\_deg}, f) = \{h, d\} $
\ENDIF
\ENDIF
\RETURN $\{h, d\}$
\end{algorithmic}
\end{algorithm}

Sometimes the degree of a polynomial is cheap to compute, for instance, if an
upper bound can be used.
%
% Rem: noun ``practice'' also in BE
It is a common practice in computational algebra to have such a degree
bound~(or \emph{sugar} value, see \citealp{GiovMNRT:91}) arising from
intermediate polynomials.
It can be generated using basic degree formulas, like
%
\begin{equation}
deg(f+g)\leq\max(deg(f),deg(g))\mfstop
\end{equation}
%
In \PolyBoRi these degree bounds are of even greater use.
%
In degree orderings they can be \utilised 
in a dual-purpose  manner: having the degree bound you
can speed up leading-term calculations, having the leading term you can improve
the degree bound. This is not the exact, original sugar strategy, but it behaves
well in practice. \Algref{alg:recursive_deg_bound} illustrates the degree
computation.
%
\begin{algorithm}
\caption{Recursive degree computation  with upper bound}
\label{alg:recursive_deg_bound}
\begin{algorithmic}
\REQUIRE $f$ Boolean polynomial, $d_{\max}$ upper bound for degree
\ENSURE $d = \deg(f, d_{\max})$
\IF{$f$ is constant}
\STATE $d = 0$
\ELSE
\IF{$\mathrm{isCached}(\deg, f, d_{\max})$}
\STATE $d = \mathrm{cache}(\deg, f, d_{\max})$
\ELSE
\STATE  $d_1 = \deg(\thenBranch(f), d_{\max} -1) + 1$
\IF{$d_1 = d_{\max}$}
\STATE $d = d_1$
\ELSE
\STATE $d = \max(d_1, \deg(\elseBranch(f), d_{\max}))$
\ENDIF
\STATE $\mathrm{cache}(\deg, f, d_{\max}) = d$
\ENDIF
\ENDIF
\RETURN $d$
\end{algorithmic}
\end{algorithm}
%
In any case,  the number~$n$ of ring variables may always be used for such an upper
bound, \ie~$\deg(f) = \deg(f, n)$.
Also caching is useful, since immediately a single call of~$\deg(f)$ 
makes~$\deg(g)$ available on the cache 
for all recursively generated subpolynomials. 
Having such a kind of cheap $\deg$-functionality available, one can formulate
\algref{alg:recursive_lead_dlex}, which only generates the leading term, but~--
unlike \algref{alg:recursive_lead_deg_dlex}~-- not the other terms of the
polynomial. 

\begin{algorithm}
\caption{Recursive leading term (degree-lexicographical)}
\label{alg:recursive_lead_dlex}
\begin{algorithmic}
\REQUIRE $f$ Boolean polynomial.
\ENSURE $h = \lead(f)$ 
\IF{$\deg(f) = 0$}
\STATE  $h = 1$
\IF{$\mathrm{isCached}(\lead, f)$}
\STATE $h = \mathrm{cache}(\lead, f)$
\ELSE
\IF{$\deg(f) = \deg(\thenBranch(f)) + 1$}
\STATE $h = \mathrm{top}(f)\cdot\lead(\thenBranch(f))$
\ELSE
\STATE $h = \lead(\elseBranch(f))$
\ENDIF
\STATE $\mathrm{cache}(\lead, f) = h$
\ENDIF
\ENDIF
\RETURN $h$
\end{algorithmic}
\end{algorithm}

Note, that similar algorithms can be formulated for the
degree-reverse-le\-xi\-co\-gra\-phi\-cal ordering with reversed variable order.
The reason for the reversion of the variables~(which  can be hidden easily 
from the user) is that the implementation can be done more
efficiently.
For instance, for computing~$\mathrm{lead\_and\_deg}$ \wrt this ordering
one just has to replace 
the strict \emph{less}-comparison in \algref{alg:recursive_lead_deg_dlex} 
by \emph{less or equal}. Analogously,
 in \algref{alg:recursive_lead_dlex},
it has to be tested for~$\deg(f)\not=\deg(\elseBranch(f)) $
instead of~$\deg(f) = \deg(\thenBranch(f)) + 1$.

\subsection{Iterators}
\label{sec:iterators}
\PolyBoRi's polynomials also provide term access. For this purpose 
iteration over all monomials was implemented in the
style of \emph{Standard Template Library}'s (STL) iterators, obtained using 
\texttt{begin()} and \texttt{end()}
member functions, like in \cite{stepanov94standard}.
Very much like a \generalisation of the pointer concept, such a kind of
\defemph{iterator} can be dereferenced to gain constant, \ie read-only, access to
the current term, and incremented to go to the next term in question. Also,
comparison with other iterators of the same type is possible. In particular,
equality with a special end marker yields the end of the iteration. This ensures
compatibility with STL algorithms, originally designed for template classes like
\texttt{std::vector} and \texttt{std::list}. 

This kind of term iterator was implemented by a stack, which stores a sequence
of references pointing to the diagram nodes. Initially, these are generated from
following the first valid path. 
%The resulting term is then stored using a temporary variable.
Incrementing the iterator is equivalent to popping the top
element from the stack as long as the corresponding nodes have invalid else-edges
only. Then the subdiagram adjacent to this edge, and also its first valid path,
is put on the stack, in order to represent the next lexicographical term. 
On dereferencing a temporary monomial holding the current term is generated.
% After popping/filling the temporary term value has to be updated subsequently.


In addition to the natural order of the underlying ZDD, more complex iterators
have been 
implemented for all supported monomial orderings. This hides the fact, that the
internal data structure is actually ordered lexicographically. Hence, we have a
sophisticated programming interface, which allows the formulation of general
procedures in the manner of computational algebra, without the need for caring
about certain properties of binary decision diagrams or the current ordering.


==> abstract.tex <==
% also included by ext_abstract!
This work presents a new framework for \Groebner basis computations 
with Boolean polynomials. Boolean polynomials can be \modell{}ed in a  rather 
simple way, with both coefficients and degree per variable lying in~$\{0, 1\}$.
%
The ring of Boolean polynomials is, however, not a polynomial ring, but rather 
the quotient ring of the polynomial ring over the field with two elements
modulo the field equations~$x^2=x$ for each variable~$x$. Therefore, the usual
polynomial data structures seem not to be appropriate for fast \Groebner basis
computations.
%
We introduce a \specialised data structure for Boolean polynomials based on 
zero-suppressed binary
decision diagrams~(ZDDs), which is capable of handling these 
polynomials more efficiently with respect to memory consumption and
also computational speed. 
Furthermore, we concentrate on high-level algorithmic aspects, 
taking into account  the new data structures as well as structural properties
of Boolean polynomials. For example, a new useless-pair criterion for
\Groebner basis computations in Boolean rings is introduced. 
One of the motivations for our work is the growing importance of formal
hardware and software verification based on Boolean expressions,
which suffer~-- besides from the complexity of the problems~--
from the lack of an
adequate treatment of arithmetic components. We are convinced  that algebraic
methods are more suited and we believe that our preliminary implementation
shows that \Groebner
bases on specific data structures can be capable to handle problems
of industrial size.


==> ack.tex <==

\begin{ack}
This work has been partly financed by the \emph{Deutsche
For\-schungs\-gemein\-schaft} (DFG) under Grand No.\ GR~640/13-1, and it has been
supported by the Rheinland-Pfalz cluster of 
excellence \emph{Dependable Adaptive Systems and Mathematical
Modelling}~(DASMOD).
In addition, the authors thank Prof.\ Gert-Martin Greuel and Prof.\ Gerhard
Pfister~(both Department of Mathematics, University of Kaiserslautern, Germany) for their encouragement.
\end{ack}

\nocite{BoCaPl97}
\nocite{Buchb65}
\nocite{GPS05}
\nocite{AlbrechtM}
%\nocite{Court02}
\nocite{Court06}
\nocite{CidMurRob05} 


==> adderblock.tex <==
Here we present an application example, which is motivated from arithmetical blocks
arising in digital systems design. An adder block unit takes two $n$-bitted
inputs~$a$ and~$b$, and computes the  sum~$s$ consisting of the lowest~$n$
bits of the addition result. In addition, another $n$~bit output~$c$ gives
a sequence of carry-overs.

In order to formulate the problem in terms of Boolean polynomials,
the Boolean variables~$a_{0}, \ldots, a_{n-1}$ and~$ b_{0}, \ldots, b_{n-1}$
are introduced for bitwise handling  of the inputs. Analogously,
the sequences~$s_{0}, \ldots, s_{n-1}$,
and~$c_{0}, \ldots, c_{n-1}$ are used to model the outgoing sums and carry bits.
%
The system can be described by the following equations
%
\begin{equation}
\begin{array}{rcl}
c_{i} + carry_i &=& 0 \\
s_{i} +a_{i}+b_{i}+ carry_i& =& 0
\end{array}
%
\quad\mbox{for}\; i=0,\ldots, n-1\mcomma
\end{equation}
%
where the~$carry_i$ denote Boolean polynomials, which are recursively defined
by setting~$ carry_{-1} = 0 $  and~$carry_i = a_{i}\cdot( b_i + carry_{i-1} )+
b_{i}\cdot carry_{i-1}$.
%
As already mentioned before,
the size of a~ZDD is very sensitive to the order of the variables.
For efficient generation and handling of the ZDD structure it is crucial to use
a variable order, which is motivated by the topology the digital system.
For this purpose, variables corresponding to outputs have to be placed before
those, marking inputs. Additionally,
obeying the recursive generation of~$carry_i$
the variables~$a_i$ and~$b_i$ have to be selected reverse alternating.

Hence, selecting~%
$a_{n-1}, b_{n-1}, a_{n-2},b_{n-2},\ldots, a_{0},b_{0}$
we obtain the ZDD structure of~$carry_i$ as shown in \figref{fig:zdd_adder}.
%
\begin{figure}[htb!]
\begin{center}
\includegraphics[scale=0.25]{zdd_adder}
\end{center}
\caption{ZDD structure representing the~$i^{\mathrm{th}}$ carry bit of an
$n$-bit adder.
%Solid/dashed connections marking then/else-edges, respectively.
\label{fig:zdd_adder}}
\end{figure}%
%
In this case the polynomial of the most significant carry bit has~$2^n-1$ terms.
%
The ususal computational approach of storing the polynomial
term-wise already causes memory problems for rather small~$n$, even in case
bit vectors are used as storage type. In contrast, the
plaited structure of the ZDD leads to a linear growth of the number of nodes
as the following theorem shows:

\begin{thm}
Let~$z_n$ be the ZDD, which corresponds to the Boolean polynomial $carry_{n-1}$
in the variables~$a_{n-1} > b_{n-1} > a_{n-2} > b_{n-2} > \dots > a_0 > b_0$, 
where~$carry_i$ is recursively defined by 
\begin{eqnarray}
carry_0 &=& a_0\cdot b_0\\
\label{eqn:carry_2}
carry_i &=& a_{i}\cdot( b_i + carry_{i-1} )+
b_{i}\cdot carry_{i-1}\mfstop 
\end{eqnarray}
Then ~$z_n$ has~$3\,n-1$ nodes.
\end{thm}

\begin{proof}
If~$n=1$ the claim in trivial. For~$n>1$  \eqnref{eqn:carry_2} adds three
new nodes to the ZDD structure of~$carry_{n-2}$, which concludes the theorem.
\end{proof}


This enables fast polynomial generation and operations during \Groebner base
computations.
%
In \PolyBoRi it is possible to use such adder structures with
thousands of bits almost instantaneously.
Although it is very unlikely, that adder blocks with bit
width larger that~128 will occur in a given design, such structures may occur in
formal verification. For instance, this is the case when properties,
which last for several clock cycles, are unrolled and reformulated in a
time-independent way. 


==> algorithm.tex <==
\section{Algorithmic Aspects in Higher Level Computations}
\PolyBoRi implements basic polynomial arithmetic as well as higher level
functions from computational algebra like \Groebner basis algorithms and normal
form computations.
%
These algorithms from computational algebra have been adjusted to the facts that:
\begin{itemize}
	\item We have a very special situation: only coefficients~0 or~1, no exponents greater than~1.
	\item The framework can only represent Boolean polynomials (which is
sufficient for the practice, since Boolean functions are equivalent to Boolean
polynomials), but not general polynomials, in particular not the field equations
themselves.
	\item Our data structures behave completely different, some operations are more costly, some are faster.
\end{itemize}
Paying attention to these points it is possible to achieve high performance using \PolyBoRi .

% \subsection{Leading Terms} moved to about_pbori.tex

\subsection{Normal Forms}
A good example for this redesign of existing algorithms is the classical normal
form computation of \algref{nf_buchberger}.
%
\begin{algorithm}
\caption{Buchberger normal form}
\label{nf_buchberger}
\begin{algorithmic}
\REQUIRE $G$ finite tuple of Boolean polynomials, $f$ Boolean polynomial.
\WHILE{$f\neq0$ and $\left(\exists g \in G: \lm(g) | \lm(f)\right)$}
\STATE $f \assign \spoly(f,g)$
\ENDWHILE
\RETURN $f$
\end{algorithmic}
\end{algorithm}
\\
A more suitable approach in \PolyBoRi would be the one of
\algref{nf_greedy}.
%
\begin{algorithm}
\caption{Greedy normal form}
\label{nf_greedy}
\begin{algorithmic}
\REQUIRE $G$ finite tuple of Boolean polynomials, $f$ Boolean polynomial.
\WHILE{$f\neq0$ and $\left(\exists g \in G: \lm(g) | \lm(f)\right)$}
\STATE $h \assign \frac{f}{\lm(g)}$ 
\hfill\COMMENT{division by remainder}
\STATE\hfill\COMMENT{\sth the result corresponds to terms in $f$ divisible by $\lm(g)$}
\STATE $f \assign f-h\boolemult g$
\hfill\COMMENT{no term of $f$ is divisible by $\lm(g)$ any more}
\ENDWHILE
\RETURN $f$
\end{algorithmic}
\end{algorithm}
\\
The latter algorithm combines many small steps. The cost of the single steps can be higher using ZDD operations, but the combined step can be done much faster.
The high cost (compared to classical polynomial representations) of these single additions might be surprising in the first moment, but can be explained quite easily.
Good normal form strategies try to select a monomial for~$g$, whenever
possible. Then of course classical structures like linked list do not need a general addition, but can simply pop the first element (term) from the list. This can be done in constant time. In fact only applying this greedy technique to the case, where~$g$ is a monomial, already gives a quite good normal form implementation in \PolyBoRi. Of course, it is a matter of heuristics to decide, when it might be better only to perform a single reduction step.

The algorithm makes more sense in the case of Boolean polynomials.
In fact, in the non-Boolean case a single reduction step can give worse results and
would be harder from the computational point of view than a reduction step in the classical Buchberger normal form algorithm.
%
\begin{exmp}
    We consider the polynomials $f=x^2+x\cdot y$ and $g=x+y$ in $\mathbb{Q}[x,y]$ with lexicographical ordering ($x>y$). Then $\spoly(f,g)=0$, but \[f+\frac{f}{\lm(g)}\cdot g=f-(x+y)\cdot g=-x\cdot y -y^2.\]
    The purpose of the the construction was to cancel all multiples of $\lm(g)$ in $f$, which includes $x\cdot y$ in this example.
    Appearently the strategy fails in this general case.
\end{exmp}
%
The following theorem shows, that in the case of Boolean polynomials (and Boolean multiplication) the situation is better.

\begin{thm}
    Let $f$, $g$ be Boolean polynomials in $\Ztwoxoneton$, $\lm(g) \divides
\lm(f)$. Then \[r:=f-\frac{f}{\lm(g)}\cdot g\] does not contain any term, which is a multiple of $\lm(g)$: $\frac{r}{\lm(g)}=0$.
    In particular, this claim holds for \[r_2:=f-\frac{f}{\lm(g)}\boolemult g\] as well. Additionally, $\support(r)\not\supset\support(\spoly(f,g))$, if $r\neq \spoly(f,g)$.
% Anm.: Vielleicht sogar $\support(r)\not\supseteq\support(\spoly(f,g))$?
% Nein, Wenn nur der Leitterm von f teilbar ist, dann passiert genau das gleiche wie bei der spoly-Bildung
\end{thm}
\begin{pf}
    We only have to show that $\frac{f}{\lm(g)} \cdot \tail(g)$ does not contain multiples of $\lm(g)$, as~$\frac{f}{\lm(g)}\cdot \lm(g)$ cancels with terms in $f$.
    W.\,m.\,a.\ $\lm(g)\neq 1$ (in this case $\tail(g)=0$). Then by elementary properties of monomial orderings no term in
$\tail(g)$ is divisible by~$\lm(g)$. On the other hand every term in
$\frac{f}{\lm(g)}$ does not contain a variable occuring in $\lm(g)$ (the maximal exponent per variable is $1$), so multiplying with this terms does not contribute to divisibility by $\lm(g)$.
    This proves the first claim.
% Anm.: Eigentlich 3 claims.
    The last claim can be shown analogously.
\end{pf}
\subsection{\Groebner Basis}

The first real \Groebner basis algorithm implemented in \PolyBoRi is an enhanced and \specialised variant of the slimgb \citep{SlimBa06}, which was implemented first in \Singular.
Slimgb is a Buchberger algorithm, which was designed to reduce the intermediate expression swell.
We call the improved version for this special case $\symmgbGFTwo$.
In particular it features a good strategy for elimination orderings~(\eg lexicographical orderings) using a special weighted length function, which not only considers the number of terms of a polynomial, but also their degree.
We will concentrate in the presentation of the results on \Groebner bases computations, as there exists a large example set and it is a task, which is  \optimis{}ed in many systems.

\subsubsection{Implementation Tricks}
The availability of ZDDs for set operations can also used for other things than
polynomial representation. For instance, having a polynomial~$p$, the search for
a polynomial~$q$ in your generations with the property, that~$\lm(q) \divides
\lm(p)$ can be implemented using set operations in the following 
way~(\algref{search_reductor}).

\begin{algorithm}
\caption{Search for reductor}
\label{search_reductor}
\begin{algorithmic}
\REQUIRE $p\neq 0$ polynomial, $G$ polynomials with $\lm (g) \not= \lm (h),
\forall g,h \in G, g\not=h$,
 $S = \{\lm(g)| g \in G \}$, \\
$\mathrm{lm2p}:S \rightarrow G$ map with $\lm(g) \mapsto g, \forall g \in G$
\hfill\COMMENT{leading term back to polynomial}
\ENSURE $D$ set of possible possible reductors
%$S$ set of leading terms,
%$\mathrm{lm2p}$ map (which maps a leading term to the corresponding ideal
%generator)
%\STATE $S \assign \{\lm(g)| g \in G \}$
%\STATE $\mathrm{lm2p}: S \rightarrow G, \lm(g) \mapsto g$ for all~$g \in G$
%\hfill\COMMENT{map back leading terms to polynomials}
%\STATE $m \assign \lm(p)$
\STATE $t \assign \set{s \in S|s \mbox{ divides } \lm(p) }$
\hfill\COMMENT{implementable as a single ZDD operation}

\STATE $D \assign \set{\mathrm{lm2p}(s)|\;\mbox{for}\; s \in t}$

\RETURN $D$
\end{algorithmic}
\end{algorithm}

This presented algorithm is supposed to be much faster than linear search, under the following (sensible) assumptions
\begin{itemize}
	\item $S$ is a large set
	\item each leading term in $S$ is unique
	\item $m$ has quite small degree compared to the number of variables
	\item D is small
	\item a call of $\mathrm{lm2p}$ has complexity $\mathcal{O}(\log_2(\#S))$
	\item $\mathrm{lm2p}$ is precomputed
\end{itemize}
This follows from the general principle, first to \minimise the set of
considered leading terms via set operations, and then to access the actual polynomial via a hash lookup.
One can also use a similar technique, when applying the product criterion.
There are many other possibilities to use the ZDDs for improving \Groebner basis computations.

\subsubsection{Criteria}
\input{criteria}


\subsection{\Groebner Proof System}

The \Groebner proof system \citep{clegg96using} is a combination of backtracking for calculation.
Traditional SAT-solvers using backtracking  split a logical expression into clauses, which have to be satisfied simultaneously~\citep{kunzetal01}.
This algorithm works the following way. On each level of the calculation a value for a chosen variable is plugged in.
If even a single clause is unsatisfiable, then the system is obviously unsatisfiable. Then the other branch (the chosen value of the opposite variable) has to be checked.

The \Groebner proof system works similar to these classical SAT-solvers. The difference is, that the criterion for a system to be obviously unsatisfiable is that a run of the Buchberger algorithm with degree bound yields one (so the ideal is the whole ring).
This algorithm has been implemented in a first experimental version. It will be a challenge for the future to find good strategies and heuristics for this very high level algorithm.




==> basic_ca.tex <==

\section{Algebraic Basics}
In this section, we recall some algebraic basics, including classical notions for
the treatment of polynomial systems, as well as basic definitions and results
from computational algebra. For a more detailed treatment of the subject see 
the book of \cite{GPS} and the references therein.

\subsection{Classical Notions}

Let $P=\Poly$ be the polynomial ring over the field $K$. A {\bf monomial ordering}
on~$P$, more precisely, on the set of monomials
$\set{x^\alpha=x_1^{\alpha_1}\cdot \ldots \cdot x_n^{\alpha_n}| \alpha \in
\mathbb{N}^n},$ is a well ordering~``$>$'' (\ie each nonempty set has a smallest
element with respect to~``$>$'')
 with the following additional property:~$x^\alpha> x^\beta \Rightarrow x^{\alpha+\gamma}>x^{\beta+\gamma}$,
for~$\gamma\in \mathbb{N}^n$.

An expression $\lambda m$ ($\lambda \in K$, $m$ a monomial) is called a {\bf term} and $\lambda$ the {\bf coefficient}. An arbitrary element $f \in P$ is called a {\bf polynomial}.

Let $f=\sum_{\alpha}c_{\alpha} \cdot x^\alpha $ ($c_{\alpha,i} \in K$) a polynomial.
Then $$\support(f) := \set{x^{\alpha} | c_{\alpha}\neq 0}$$ is called the {\bf support} of $f$.


Furthermore $\lm(f)$ denotes the {\bf leading monomial} of~$f$, the biggest monomial occurring in $f$ \wrt ``$>$'' (if $f \neq 0$).
The corresponding term is denoted by $\lt(f)$ and the coefficient by $\lc(f)$. Moreover, we set 
$$\tail(f):=f-\lt(f).$$
If \mbox{$F \subset P$} is any subset, $L(F)$ denotes the {\bf leading ideal} of~$F$, \ie the ideal in $P$ generated by $\set{\lm(f)|f \in F\backslash \set{0}}$. The S-Polynomial of $f,g \in P\backslash \set{0}$ with $\lm(f)=x^\alpha$, $\lm(g)=x^\beta $ is denoted by
$$\spoly(f,g) := x^{\gamma-\alpha} f- \frac{\lc(f)}{\lc(g)} x^{\gamma-\beta} g,$$ where  $\gamma=\lcm(\alpha,\beta):=(\max(\alpha_1, \beta_1), \ldots, \max(\alpha_n, \beta_n))$.
Recall that $G \subset P$ is called a {\bf Gr\"obner basis} of an ideal $I\subset P$, if $\{\lm(g)|g \in G\backslash \{0\}\}$ generates  $L(I)$ in the ring $P$ and $G \subset I$.

%Furthermore $\V(I)$ denotes the common zeroes of a set of polynomials $I$.

\begin{defn}[Standard representation]
Let \mbox{$f, g_1, \ldots g_m \in P$}, and let \\
\mbox{$h_1, \ldots , h_m \in
  P$}. Then 
$$f = \sum_{i=1}^{m}h_i \cdot g_i  \in K[x_1, \ldots, x_n],$$
is called a standard representation of~$f$ with respect to $g_1, \ldots ,g_m$,
if
$$\forall i: h_i\cdot g_i=0 \text{ or otherwise } \lm(h_i \cdot g_i) \leq \lm(f)\,\mbox{.} $$
\end{defn}
% ----------------------------------------------------------------
\noindent
The classical product criterion of Buchberger \citep{BBcrit} reads as follows:
%%%%%%%%%%%% literature
\begin{lemma}[Product criterion]
Let $f,g \in \Poly$ be polynomials.
If the equality~$\lm(f) \cdot \lm(g)=\lcm(\lm(f),\lm(g))$ holds, then~$\spoly(f,g)$ has a standard representation \wrt $\{f,g\}$.
\end{lemma}

\begin{defn}[Elimination orderings]
Let $R=K[x_1,\ldots, x_n, y_1, \ldots y_m]$. An ordering~``$>$'' is called an elimination ordering of $x_1, \ldots, x_n$, if $x_i>t$ for every monomial~$t$ in~$K[y_1, \ldots, y_m]$ and every $i=1,\ldots,n$. 
\end{defn}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%This section should be unnecc. for PolyBoRi
\subsection{$t$-Representations}
\label{t-rep}
% ----------------------------------------------------------------

There is an alternative approach to standard representations formulated in \citep{Bec93} and used in \citep{F4}, which \utilises the notion of $t$-representations. While this notion is mostly equivalent to using syzygies, it makes the correctness of the algorithms easier to understand.
% ----------------------------------------------------------------
\begin{defn}[$t$-representation]
\ifx\itwmrep\undefined\relax\else{~\\}\fi
Let $t$ be a monomial, $f, g_1, \ldots g_m \in P$, $h_1, \ldots , h_m\in P$. Then
$$f = \sum_{i=1}^{m}h_i \cdot g_i  \in P$$
is called a $t$-representation of $f$ with respect to $g_1, \ldots ,g_m$
if
$$\forall i: \lm(h_i \cdot g_i) \leq t \text{ or } h_i\cdot g_i=0\,\mbox{.}$$
\end{defn}
% ----------------------------------------------------------------
\begin{exmp}
~

\begin{itemize}
\item Let the monomials of $P$ be lexicographically  ordered
($x > y $) and let
$$t=x^5y^5, g_1= x^2, g_2=x^5-y, f=y$$
\item Then $f=x^3 g_1 - g_2$ is a $x^5y^5$-representation for $f$.

\item Each standard representation of $f$ is a $\lm(f)$-representation.
\item For $t<\lm(f)$ $t$-representations of $f$ do not exist.
\end{itemize}
\end{exmp}
% ----------------------------------------------------------------
\noindent
{\bf Notation:} Given a representation $p=\sum_{i=1}^{m}h_i\cdot f_i$ with
respect to
a family of polynomials~$f_1, \ldots f_m$, we may shortly say that $p$ has a
{\bf nontrivial $t$-representation}, if a $t$-representation of $p$ exists with
$$t<\max\{\lm(h_i\cdot f_i)\vert h_i \cdot f_i\neq 0\}.$$ 
For example, $\spoly(f_i,f_j)$ has a nontrivial $t$-representation if there
exists a representation of $\spoly(f_i, f_j)$ where the summands have leading terms smaller
than $$\lcm(\lm(f_i), \lm(f_j)).$$



\begin{theorem} 
%Let $F=(f_1, \ldots, f_k)$, $f_i \in \Poly$, be a polynomial system.
%For $i$, $j$ define $m_{i,j}$ as follows: If $\lm(f_i)={x}^{\alpha}$, $\lm(f_j)={x}^{\beta}$, then define $m_{i,j}=\lcm({x}^{\alpha}, {x}^{\beta})/{x}^{\alpha}$.
%The following are equivalent:
%\begin{enumerate}
%\item $F$ is a Gr\"obner basis of $\langle F \rangle_\Poly$
%\item Set $$M:=\set{(i,j)|1\leq i<j\leq \#F}.$$
%Then, for any subset $J \subset M$ with
%
%
%\begin{align*}\langle \{m_{i,j}\cdot e_i |(i,j) \in J\} \rangle_\Poly &=\\  \langle \{m_{i,j}\cdot e_i |(i,j) \in M\}\rangle_\Poly & \subseteq \\ \Poly^r\end{align*} 
%$\spoly(f_i,f_j)$ has a nontrivial $t$-representation \wrt F (i.e. for some \\
%$t<\lcm(\lm(f_i),\lm(f_j))$) $\forall (i,j) \in J$.
%\end{enumerate}
Let $F=(f_1, \ldots, f_k)$, $f_i \in \Poly$, be a polynomial system. If for each $f$, $g$ $\in F$ $\spoly(f,g)$ has a nontrivial $t$-representation \wrt $F$, then $F$ is a Gröbner basis.


\end{theorem}
\begin{pf}
For a full proof see \citep{Bec93}. A more sophisticated version of this theorem can be formulated and proven analogously to ~\citep[p. 142]{GPS}.
\end{pf}

%\begin{theorem}[extended product criterion]
%Let $f=h\cdot f'$, $g=h \cdot g'$ and $f, g, f', g'\in P^r$, $h \in P$ be polynomials lying completely in the same module component.
%If $\lm(f') \lm(g')=\lcm(\lm(f'),\lm(g'))$ then $\spoly(f,g)$ has a standard representation \wrt $\{f,g\}$.
%\end{theorem}
%\begin{pf}
%As the product criterion holds for $f'$, $g'$, there exist polynomials $\lambda$, $\mu$, s.t.\ $\spoly(f',g')=\lambda f'+ \mu g'$ is a standard representation. Then also
%$\spoly(f,g)=\lambda f + \mu g$
%is a standard representation.
%\end{pf}

%\begin{rem} In practice the extended product criterion will be applied only to the case where the common factor $h$ is a monomial.
%In this case it is very fast to check: for each polynomial $f$ one computes $m_f$, the monomial gcd of all its terms. Considering the pair $f$, $g$ one only has to take the gcd of the two monomials $m_f$, $m_g$.
%However in certain situations (e.g. cryptographic systems) one can easily detect
%some other factors. The speedup can be significant.
%This criterion, though simple, seems to have been overlooked so far.
%\end{rem}
%
%\noindent
%The following is a reformulation of the classical Buchberger's chain criterion for $t$-re\-pre\-sen\-ta\-tions.
%\begin{theorem}[$t$-chain criterion]
%Let G be a list of polynomials, and let
%$f_1,f_2, \ldots , f_m\in G$ with leading monomials involving the same module component, $\lm(f_i)=x^{\alpha_i} e_j$, such that
%$$\forall i: x^{\alpha_i}\vert \lcm(x^{\alpha_1},x^{\alpha_m}).$$
%Assume that for all $i \in \set{1, \ldots, m-1}$, one of the two following conditions holds:
%\begin{enumerate} 
%\item $\spoly(f_i,f_{i+1})$ has a (nontrivial) $t$-representation for some
%  monomial\\
% $t<\lcm(\lm(f_i),\lm(f_{i+1}))$ with respect to G.
%
%\item $x^{\alpha_i} \cdot x^{\alpha_{i+1}} \vert \lcm(x^{\alpha_1},x^{\alpha_m})$ and $f_i$, $f_{i+1}$ lie completely in the same component.
%\end{enumerate}
%Then $\spoly(f_1,f_m)$ has a (nontrivial) $t$-representation for some monomial\\
% $t<\lcm(\lm(f_1),\lm(f_m))$ with respect to G.
%\end{theorem}
%
%\noindent
%This generalizes results in \citep{Bec93}, the trivial syzygy approach is inspired by \citep{F5}.
%\begin{pf}
%Without loss of generality we may assume that all $f_i$ are normalized. Then
%\begin{eqnarray*}
%\lefteqn{\spoly(f_1,f_m)}\hspace{0.5cm}\\
%&=&t_1 \cdot \spoly(f_1,f_2)+  t_2 \cdot \spoly(f_2,f_3) + \ldots + t_{m-1}
%\cdot \spoly(f_{m-1},f_m)
%\end{eqnarray*}
%where $$t_i=\lcm(\lm(f_1),\lm(f_m))/\lcm(\lm(f_i),\lm(f_{i+1})).$$
%%If each summand has a nontrivial $t$-representation,
%%then the sum has a nontrivial $t$-representation.
%Therefore, it remains to show, that each summand has nontrivial $t$-re\-pre\-sen\-ta\-tion (precisely some $t<\lcm(\lm(f_1),\lm(f_m))$).
%
%If condition 1 holds, then the multiplication by the monomial $t_i$ gives just a good t, which satisfies our condition. 
%In the second case one has the trivial syzygy 
%$p_i\cdot f_{i+1}-p_{i+1}\cdot f_i=0$ (using $f_i=p_i\cdot e_j$, $f_{i+1}=p_{i+1}\cdot e_{j}$). Therefore
%$$\lm(p_{i+1})\cdot f_i-\lm(p_i)\cdot f_{i+1}=\tail(p_i)\cdot
%f_{i+1}-\tail(p_{i+1}) \cdot f_i.$$ If condition (2) holds, we have only to
%multiply both sides with $$\lcm(x^{\alpha_i}, x^{\alpha_m}) /
%(x^{\alpha_i}\cdot x^{\alpha_{i+1}}).$$
%\end{pf}


==> blockorder.tex <==
% store maybe for the use at ISSAC or so...
\begin{algorithm}[htb]
\caption{Polynomial degree  $d = \deg(f)$}
\label{alg:recursive_deg}
\begin{algorithmic}
\REQUIRE $f\in \Bool$

\IF{$f$ is constant}
\STATE  $d = 0$
\ELSE
\IF{$\mathrm{isCached}(\deg, f)$}
\STATE $d =\mathrm{cache}(\deg, f)$
\ELSE
\STATE $\mathrm{cache}(\deg, f) =
   d=\max(\,\deg(\thenBranch(f))+1, \deg(\elseBranch(f))\,)$
\ENDIF
\ENDIF
\RETURN $d$
\end{algorithmic}
\end{algorithm}

\subsubsection{Block orderings}

Another important feature for \Groebner packages is the availability of
orderings, which are composed of blocks of degree orderings.
The procedures presented in \secref{sec:deg_ord}
can be extended to this case.
The active ordering
has to be equipped with an array of decision variables~$x_{i_1} >x_{i_2} >
\cdots > x_{i_r}$  marking the start of the second, third, \ldots,
$(r+1)^{\mathrm{th}}$  block, respectively.
%
The block degree \wrt the first block can easily be computed by extending
\algref{alg:recursive_deg} in the following way: in addition to the condition,
that the polynomial \emph{$f$ is constant}, the degree calculation is also
terminated and set to zero, when~$\mathrm{top}(f)$ reaches a decision variable,
which is less or equal to~$x_{i_1}$. \Algref{alg:recursive_block_deg}
illustrates this procedure in whole.
%
%
\begin{algorithm}
\caption{Polynomial block-degree  $d = \blockdeg(f, x)$}
\label{alg:recursive_block_deg}
\begin{algorithmic}
\REQUIRE $f\in\Bool$, $x$ Boolean variable marking next block

\IF{$f$ is constant \textbf{or} $\mathrm{top}(f) \leq x$ }
\STATE  $d = 0$
\ELSE
\IF{$\mathrm{isCached}(\blockdeg, f, x)$}
\STATE $d =\mathrm{cache}(\blockdeg, f, x)$
\ELSE
\STATE $d = \max(\,\blockdeg(\thenBranch(f),x)+1,
        \blockdeg(\elseBranch(f),x))\,)$
\STATE $\mathrm{cache}(\blockdeg, f, x) = d$
\ENDIF
\ENDIF
\RETURN $d$
\end{algorithmic}
\end{algorithm}



For instance, consider the leading term computation for
degree-lexicographic blocks.
The sequence of block borders can easily be encoded as the
monomial~$m=x_{i_1}\cdot x_{i_2} \cdot \ldots\cdot x_{i_r}$.
Like in the case without blocks, one starts to follow the path
of largest degree, but~-- in contrary~-- here we have to deal with the
block degree of the first block.
%
When the beginning of the next block is reached~$m$ is replaced
by~$\thenBranch(m)$. This ensures that \algref{alg:recursive_block_deg}
for computing the first block degree can  be reused for successive blocks.
%
\begin{algorithm}
\caption{Block degree-lexicographical leading term $h = \lm(f, m)$}
\label{alg:recursive_lead_blockdlex}
\begin{algorithmic}
\REQUIRE $f\in\Bool$, $m$ Boolean monomial marking block starts.
\IF{$m = 1$}
\STATE $h = \lm(f)$
\ELSE
\STATE $x = \mathrm{top}(m)$
\IF{$\mathrm{top}(f)   \leq  x $  }
\STATE $h = \lm(f, \thenBranch(m))$
\ELSE
%
\IF{$\mathrm{isCached}(\lm, f, m )$}
\STATE $h =\mathrm{cache}(\lm, f, m)$
\ELSE
\IF{$\blockdeg(f, x) =
  \blockdeg(\thenBranch(f), x) + 1$}
\STATE $h = \mathrm{top}(f)\cdot\lm(\thenBranch(f), m)$
\ELSE
\STATE $h = \lm(\elseBranch(f), m)$
\ENDIF
\STATE $\mathrm{cache}(\lm, f, m) = h$
\ENDIF\ENDIF
\ENDIF
\RETURN $h$
\end{algorithmic}
\end{algorithm}
%
Again, a suitable recursive formulation which enables caching can
improve the performance significantly.
For more details see \algref{alg:recursive_lead_blockdlex}. 


==> criteria.tex <==


Criteria for keeping the set of critical pairs in the Buchberger algorithm small are central part of \Groebner basis algorithms. In most implementations the chain criterion and product criterion  or variants of them are used.

These are of quite general type. This leads to the question, whether we can
formulate new criteria for our particular case. There are two types of pairs to
consider: Boolean polynomials with field equations, and pairs of Boolean polynomials.
We concentrate on the first kind of pairs here.

\begin{thm}
	Let $f$ be a Boolean polynomial in $\Ztwoxoneton$, $f=l\cdot g$, $l$ a polynomial with linear leading term $x_i$, $g$ a polynomial. Then $\spoly(f,x_i^2+x_i)$ has a nontrivial $t$-representation against the system consisting of~$f$ and the field equations.
\end{thm}
\label{linear-factor-criterion}
\begin{pf}
	First, we consider the case~$g=1$. In this situation the following formula holds: $\lm(f)=x_i$.
	Let~$r$ be a reduced normal form of $\spoly(f,x_i^2+x_i)$ against~$f$ and the field equations.
	Then~$r$ is (tail) reduced, so it is a Boolean polynomial and irreducible against~$f$, so $x_i$ does not occur.
	In particular considered as a Boolean function it is independent from the value of $x_i$.

	Since~$r$ is a linear combination of~$f$ and field equations (which are
zero considered as Boolean functions) we get: $$r(x_1,\dots,x_n)=1 \Rightarrow f(x_1,\dots,x_n)=1.$$
%
	Now, we assume that $r\not=0$. As a nonzero Boolean polynomial
corresponds to a nonzero Boolean function, we know, that there exist
$v_1,\ldots,v_n \in \set{0,1}$, subject to~$g(v_1,\ldots,v_n)=1$.  The above
implication gives~$f(v_1,...,v_n)=1$.
 
	Then we can change the value of $x_i$ without affecting the value of $r$ $$r(v_1,\ldots,v_i+1,\ldots,v_n)=1,$$ but $$f(v_1,\ldots,v_i+1,\ldots,v_n)=0,$$ as $x_i$ only occurs in the one term $x_i$ of $f$. This contradicts the above implication between $r$ and $f$. So $r=0$ and $\spoly(f,x_i^2+x_i)$ has a standard representation.
	
	Now, we consider a general Boolean polynomial $g$.
	$\spoly(l,x_i^2+x_i)$ has a standard representation against $l$ and the field equations:
$$\spoly(l,x_i^2+x_i)=\sum_{j=1}^n h_j \cdot x_j^2+x_j+\alpha\cdot l\,\mbox{,}$$
for polynomials $\alpha,h_j$ ($j \in \set{1,\ldots,n}$): 
%
$$x_j^2\cdot  \lm(h_j)\leq \lm(\spoly(l,x_i^2+x_i))<x_i^2\,\mbox{,}\quad 
  \lm(\alpha \cdot x_i)<x_i^2\,\mbox{.}$$
%
	We multiply this equation by $g$ and get by that fact, that $x_i$ does not occur in $g$:
%
\begin{eqnarray*}
\spoly(l\cdot g,x_i^2+x_i) &=& \spoly(l\cdot g,g\cdot x_i^2+x_i)-\tail(g)\cdot
(x_i^2+x_i)\\
                   &=& g \cdot \spoly(l,x_i^2+x_i)-\tail(g)\cdot (x_i^2+x_i).
\end{eqnarray*}
%
Using the standard representation for $\spoly(l,x_i^2+x_i)$ from above, both summands have a $t$-representation for a monomial~$t<x_i^2 \cdot \lm(g)$, so we also get a nontrivial $t$-representation in the sum.
%
\end{pf}

\begin{rem}
	The polynomials $l$ and $g$ are indeed Boolean polynomials, as a Boolean polynomial only factors in Boolean polynomials~(this can be seen using degree formulas).
	Together with the product criterion, we get, that we have only to consider pairs of Boolean polynomials $f$ with field equations for variables $x$, which do not occur in an irreducible nonlinear factor of $f$.
	In the above proof, we make use of the fact, that we only consider well orderings, when claiming, that $x_i$ does not occur in the tail of $f$.
\end{rem}	


==> ext_abstract.tex <==


\begin{tabular}{@{\bfseries}ll}
Title &
\PolyBoRi: A framework for Gröbner basis computations with\\[-1ex] 
& Boolean polynomials\\
Authors &
{Michael Brickenstein} \\[-1ex] 
 & Mathematisches Forschungsinstitut Oberwolfach \\[-1ex] 
 &Oberwolfach, Germany\\
&
{Alexander Dreyer}\\[-1ex] 
&Fraunhofer Institute for Industrial Mathematics~(ITWM)\\[-1ex] 
 & Kaiserslautern, Germany
\end{tabular}

\section*{Extended Abstract}

Normal forms for Boolean expressions play an important role in various
application areas like cryptography, logic, and formal verification of digital
systems. In fact, they are at the heart of modern model checking for 
verification of software and hardware design and it is believed that its
industrial applications will grow significantly in the next few years.

Boolean expressions and functions can be restated in
terms of polynomial systems over the field with two elements~$\mathbb{Z}_2$. 
Boolean functions can be identified with the  so-called 
\defemph{Boolean polynomials} which are subject to restrictions
given by field equations~$x_\nu^2 = x_\nu$ for all given variables~$x_\nu$.
% 
Although Gröbner bases have already become a standard tool for
treating polynonomial systems, 
current implementations have not been capable of 
satisfyingly handling
Boolean polynomials from real-world applications yet.

\input{abstract}

\subsection*{Introduction}
After a brief introduction about the intention of this work and possible
application areas, we concentrate on \defemph{formal verification}, which is a
key application of our work. 
%
During the design process of digital systems it is a major goal to have an
automated and dependable way of finding errors in a given layout, before a
prototype is build actually. Classical methods for design validation include
simulation of the system with respect to suitable input stimuli as well as tests
based on emulations. These cannot cover the
overall behaviour of a proposed implementation. In contrary, \emph{exact}
mathematical methods have the ability of automatic verification of presumed
properties.  Here, methods from computer algebra
may lead to generic procedures, which can handle systems, which are not yet
verifiable.



\subsection*{Boolean Polynomials as Sets}
We start with a motivation of the major data structure of the
C++ library \PolyBoRi for \emph{Po}lynomials over \emph{Bo}olean
\emph{Ri}ngs. 
%
Because of its simplified term structure a Boolean polynomial~$p$ can be
identified with a~(unique) subset~$S_p$ of the power set over the set of all
variables. For this polynomial and set the
relation~$p=\sum_{s\in S_p} \left( \prod_{x_\nu \in s}x_\nu \right)$ holds.
It is reasonable to assume that~$S_p$ is sparse initially, \ie
the set is only a small subset of the power set. 
Even the term can be considered to be sparse, as usually 
quite few variables occur in a monomial.
Consequently, the strategies of the used algorithms have to be tuned in
such a way, that this kind of sparsity is preserved.

Next, the notion of the \defemph{zero-suppressed binary decision
diagram}~(ZDD) will be presented~\citep{Ghasemzadeh05, berardetal01}. It is a special variant of binary decision
diagrams, which can efficiently
be used to store sparse subsets, like the set~$S_p$ mentioned above. 
%
This approach is compared with earlier attempts of using ZDDs for representing
more general polynomials \citep{Minato95}. 
In the Boolean case, a more general mapping from
polynomials to decisions diagram occurs. Also, this includes the polynomial
arithmetic, since here, operations can immediately be implemented using
combinations of primitive set operations.  This is mainly due to the fact, that
we only have to deal with trivial coeffcients and degrees. These do not need a
costly encoding, which would introduce a plenty of new decision variables to the
ZDDs. 
Using this simplified model, we were able to implement more advanced operations, which are related to monomial orderings and essential for the computation of Gröbner bases.

In addition, the idea is considered in the context of the meta
approach of \cite{coudert92implicit}: 
A number of~$n$ Boolean variables yield~$2^n$
possible configurations. 
Enumerating all valid solutions with respect to rather simple
relations leads to large and dense sets. Since those
sets cannot be handled efficiently, it had been suggested to store and
manipulated those relations, which implicitly define the sets.
%
In the language of computer algebra, the implicit relations are exactly the
systems of Boolean polynomials decribed in this paper.

\subsection*{Algebraic basics}
After this, we give some algebraic basics, starting with the  classical
notions of \defemph{polynomial}, \defemph{monomial ordering}, \defemph{leading
monomial}, \defemph{term}, and \defemph{ideal}, as well as the definition of the
\defemph{spoly} and the \defemph{Gröbner basis}. 
We also recall the \defemph{standard representation} of a polynomial and
Buchberger's \defemph{product criterion}~\citep{BBcrit}. 

Then the notion of \defemph{t-representation}s is stated as an alternative to
standard representations~\citep{Bec93, F4}. 
While it is mostly equivalent to using
syzygies, it makes the correctness of the algorithms easier to understand.
For the definition, 
let~$t$ be a monomial, $f, g_1, \ldots g_m$, and  $h_1, \ldots , h_m$ are
polynomials. Then the representation
$f = \sum_{i=1}^{m}h_i \cdot g_i$
is called a t-representation of~$f$ with respect to $g_1, \ldots ,g_m$
if
$\lm(h_i \cdot g_i) \leq t \text{ or } h_i\cdot g_i=0$ for all~$i$.
%
Nontrivial t-representations~(\ie if~$t<\max\{\lm(h_i\cdot f_i)\vert h_i \cdot f_i\neq 0\}$) can be used to decide whether a given generating
system is actually a Gröbner basis.  

\subsection*{The \PolyBoRi Framework}
The next section is dedicated to the \PolyBoRi C++ library framework.
It provides high-level
data types for Boolean polynomials and monomials, exponent vectors, as well as
for the underlying polynomial rings.
%
ZDDs are used as internal storage type, but hidden from the user. 
%
In addition, basic polynomial operations
have been implemented and associated to the corresponding operators. 
In order to enable efficient implementation, 
these operations were reformulated in terms of set operations, which are
compatible with the ZDD approach.

In particular, we purpose a recursive formulation of the procedures, which
enables the caching of intermediate results. In case of recurring common
sub-structures, cache look-up of the previous results can speed up computations.
It is very useful during Gröbner base
computations, where likewise polynomials occur quite often.
%
This also applies to other classical functionality like degree computation and
leading term computations, which is  currently
available for a selection of monomial orderings.

For all of these, iterators in the style of the \emph{Standard Template Library}
have been implemented, which allow term access with
respect to the ordering. This hides the fact, that the
internal data structure is actually ordered lexicographically. Hence, we have a
programming interface, which allows the formulation of general
procedures in the manner of computational algebra, without the need for caring
about internal issues.
%
A complete Python interface allows for parsing of complex polynomial systems, 
and enables sophisticated  strategies for Gr{\"o}bner base
computations.

\subsection*{Algorithmic Aspects in Higher Level Computations}
Second to last, we give some explanations about algorithms implemented in
\PolyBoRi. It is useful to obeye the strengths and weaknesses of ZDDs as
data structure. Therefore, classical implementations are not transfered
one-to-one to our environment, but have to be tuned accordingly. 
The computation of leading terms for degree-orderings can be made more
efficient, in case that upper bounds for the degree of the polynomials are
available from previous calculations. 

Also, a greedy variant of Buchberger's normal form algorithm is designed. Its
main advancement is the combination of many likewise spoly computations in one
combined step. Since repeated search for the same leading monomial in the
underlying decision diagrams and addition is expensive, it is more suitable to
eliminate as much terms as possible at once. Hence, during normal form
computations spoly calculation between two polynomials~$f$ and~$g$, is replaced
by computing~$f- h\cdot g$, with~$h=f/\lm(g)$ (division with remainder). The
result is not divisible by~$\lm(g)$, which saves additional iterations.
%
Especially for monomial~$g$ this can be done much more efficient on ZDDs than
doing a lot of single steps one after another.


The first real Gröbner basis algorithm implemented in \PolyBoRi is an enhanced
and specialized variant of the \Singular's \defemph{slimgb}~\citep{GPS05, SlimBa06}. 
Slimgb is a Buchberger
algorithm, which was designed to reduce the intermediate expression swell.  In
particular, it features a good strategy for elimination orderings~(\eg lex.\
orderings) using a special weighted length function, which not only considers
the number of terms of a polynomial, but also their degree.

For this algorithm some implementation tricks are show, which can be applied, if
ZDDs are available for set operations. For instance, the search for a reductor
is illustrated. First, the set of possible leading terms is minimized via
set operations. After this, matching polynomials can be accessed using a hash
look-up. 

Also, criteria for keeping the set of critical pairs in the Buchberger algorithm
small are part of the considerations. The classical chain and product criteria
are of general type, but for the special case of Boolean polynomials, an
additional condition is introduced and proved:
If~$f$ is a Boolean polynomial in $\Ztwoxoneton$, $f=l\cdot g$, $l$ a polynomial
with linear leading term $x_i$, $g$ a polynomial, then $\spoly(f,x_i^2+x_i)$ has a nontrivial t-representation against the system consisting of~$f$ and the field equations.

Additionally, a  \defemph{Gröbner proof system}~\citep{clegg96using} 
has been implemented in a first experimental version. It  splits logical expressions into clauses, which have to be satisfied simultaneously.
If even a single clause is unsatisfiable, then the system is obviously
unsatisfiable. On each level of the calculation, both true and false are plugged
in subsequently as Boolean values for a chosen variable. Satisfiability is
checked independently on the resulting branches.

\subsection*{Results}
Finally, we evaluate the implementation using some benchmark examples from current research problems in formal verification and algebraic crypto analysis.
%
In comparison with other computer algebra systems, we conclude, 
that the implemented Gröbner basis algorithm in
\PolyBoRi offers a good performance combined with low memory consumption.  Part
of the strength in directly computing Gröbner bases (without walk or similar
techniques) is inherited from the slimgb algorithm in \Singular.  The data
structures provide a fast way to rewrite polynomials, which might be of bigger
importance than sparse strategies in the presented examples.
%
It can be
seen, that the advantage of \PolyBoRi grows with the number of variables. For
many practical applications this size will even bigger. We are very confident,
that it will be possible to attack some of this problems in future by using more
specialized approaches. This will be a key point in the development of \PolyBoRi
to facilitate problem specific, high performance solutions.



==> form_veri.tex <==
%\subsection*{Formal Verification}
Even though it is not essential for the present paper, the reader may be
interested in the following short description of one important application:
\defemph{Formal verification}
is a key challenge during the design process of digital
systems. The goal is to have an automated and dependable way of finding errors
in a given layout, before a prototype is built.
See also \citep{McMillan, HachtelBook, kunzetal01} for more details.

Classical methods for design validation include the simulation of the system
with respect to suitable input stimuli as well as tests based on emulations,
which use simplified prototypes.  The latter may be constructed using field
programmable gate arrays~(FPGAs).\-
%
Due to a large number of possible settings, these approaches cannot cover the
overall \behaviour of a proposed implementation.  In the worst case, a defective
system is manufactured and delivered, which might result in a major product
recall.
%% erst mal raus, meint GMG.
% Indeed this
%has happened, when the Intel Pentium bug was overlooked, which resulted in a
%major product recall~\citep{pratt95anatomy}. 

In contrast, formal verification methods are based on \emph{exact} mathematical
methods for automated proving of circuit properties. 
%
In this context several approaches like SAT-solving, graph representation of
Boolean functions, and (timed) finite automata are already in use for bringing a
designer's concept into agreement with the required
specifications.  
%
Here, formal methods have the ability to disclose unexpected side-effects
early in the design process, and also they may show that certain short-hand
assumptions are really true for all input patterns and states.

The ability of checking the validity of a proposed design restricts the design
itself: a newly introduced design approach may not be used for an implementation
as long as its verification cannot be ensured.
%
In particular, this applies to digital systems consisting of combined logic and
arithmetic blocks, which may not be treated with \specialised approaches.
%
Here, dedicated methods from
computer algebra 
may lead to more generic procedures, which help to fill the design gap.



==> interpolation.tex <==
\providecommand{\Groebner}{Gr\"obner\xspace}
% Rem: Vorschlag: kürzere Überschrift, und ``The Task'' weglassen
\section{Boolean Interpolation}

%\section{Interpolation of Boolean functions}
%\subsection{The Task}
% Rem.: Vielleicht die partial functions als $f: (Z\cup O) \rightarrow \Ztwo$
% definieren, und die f_p unten erst als Erweiterung $f_p: \Ztwo^n \rightarrow
% \Ztwo$ ? 
%
A partial Boolean function~$f: \Ztwo^n \rightarrow \Ztwo$ can defined defined by two disjoint subsets~$Z$,\,$O$ of~$\Ztwo^n$, where~$f(o)=1$ and~$f(z)=0$ for each~$z \in Z$, $o \in O$.
Given~$O$ and~$Z$ we can also denote~$f$ by~$b_Z^O$.
%
The word \emph{partial} implies, that $Z \cup O$ can be a proper subset of~$\Ztwo^n$.

Given two partial Boolean 
functions~$b_{Z_1}^{O_1}, b_{Z_2}^{O_2}: \Ztwo^n \rightarrow \Ztwo$. We define
the sum~$(b_{Z_1}^{O_1}+b_{Z_2}^{O_2}): \Ztwo^n \rightarrow \Ztwo$ as
%
$x\mapsto b_{Z_1}^{O_1}(x)+b_{Z_2}^{O_2}(x)$ for all~$x \in (Z_1\cup O_1) \cap (Z_2 \cup O_2)$.



For this partial function definition we want to find a Boolean polynomial~$p$,
where the associated function~$f_p$ is a \specialisation of~$f$, \ie~$f_p(x)=f(x)$ for each~$x \in O \cup Z$.

Algorithms to calculate this interpolation can be compared in performance and compactness of the result.
Moreover, it would be worthwhile, if the output can be defined by a simple mathematical property.

In the following, we present a method with very compact result, where the result is lexicographically reduced \wrt the vanishing ideal of~$O\cup Z$. In this way it can also be reinterpreted as fast normal form computation against this ideal.

A partial Boolean function can be represented as a pair of two ZDDs $Z$ and $O$ in the following way.
A point $v$ in $\Ztwo^n$ can be identified in the same way like the monomial
$x^v$ with a subset of ${1, \ldots, n}$ as~$v \leftrightarrow \set{i|v_i=1}$.
In the same way we can identify a set of points with a subset of the power set of~$\set{1, \ldots, n}$ or a ZDD.

In this spirit, the addition of two partial Boolean functions could be expressed as follows in terms of ZDD operations:
$$D=(Z_1\cup 0_1)\cap (Z_2 \cup O_2)$$
$$(b_{Z_1}^{O_1}+b_{Z_2}^{O_2}) = 
b_{(Z_1\cap Z_2)\cup (O_1\cap O_2)}^{(\symmdiff{O_1}{O_2})\cap D}\mfstop$$


\subsection{Encoding}
A vector $v=(v_1, \ldots,v_n) \in \Ztwo^n$ can be encoded just as the Boolean monomial $x^v$ by the set containing all indices $i$, where $v_i \neq 0$. So, analogously to polynomials a subset of~$\Ztwo^n$ can be translated a subset of the power set of $\set{1, \ldots, n}$.
% Rem.: Maybe better ``subset of the power set of ...'' ja.
%
Using this encoding, we obtain a compact data structure for these
kinds of sets, which shares some common parts of the vectors. 
The latter may be treated simultaneously by the a recursive method.
Also, efficient caching of intermediate results for reuse is possible.

\subsection{Zeros of a Boolean polynomial}
In this section, we introduce an algorithm for computing the zeros of a given
Boolean polynomial in a~(possibly proper) subset of~$\Ztwo^n$.
For illustration a single vector~$v=(v_1, \dots,v_n)$ in~$\Ztwo^n$ is considered.
%
One may define a sequence by setting~$p_{0}=p$, and subsequently substituting
all variables by its corresponding Boolean value in~$v$ as~$p_i =
p_{i-1}|_{x_i=v_i}$.
%
This terminates ultimately in~$0$ or~$1$. Hence, it proves whether~$v$ is
a zero of~$p$ or not.  
For a set of vectors, one could do this evaluation element-wise, but this \naive
approach is not suitable for large sets.
%
In contrast, using the encoding proposed above, some common parts of the
vectors may be treated simultaneously.  Again,  the
resulting subset may be encoded as a decision diagram ``on the fly''
as \algref{alg:recursive_zeros} shows.





\begin{algorithm}
% Rem.: ``|'' in textmode becomes something like --
\caption{Recursive Zeros: $\zeros(p,S)$}
\label{alg:recursive_zeros}
\begin{algorithmic}

\REQUIRE Boolean polynomial $p$, $S$ set of points in $\Ztwo^n$\\ represented as
ZDDs
\ENSURE $\zeros(p,S)=\{s\,|\,s \in S\;\text{and}\; p(s)=0\}$

\IF{$p = 0$}
\RETURN $S$
\ENDIF
\IF{($p = 1$) or ($S=\emptyset$)}
\RETURN $\emptyset$
\ENDIF
% Q.: ZDD(\{\{\}\})} entspricht {(0, ...,0)}, vielleicht anmerken?
\IF{$S=\ZDD(\{\emptyset\})$}
%\COMMENT{$S$ consists only of the zero vector}
\IF{$p$ has constant part}
\RETURN $\emptyset$
\ELSE
\RETURN $S$
\ENDIF
\ENDIF
\STATE \COMMENT{As from now $p, S$ are certainly non-constant ZDDs.}
% Re.: Hier implizit top(0)=top(1) = infinity oder max_index. (Nach reichlicher
% Überlegung: Ist aber eigentlich von der Definition her klar, da dann min(leere
% Menge) unendlich. Vielleicht trotzdem irgendwo anmerken?)
\WHILE{$\zddtop(p)<\zddtop(S)$}
\STATE{$p = \zddelse(p)$}
\ENDWHILE
\STATE {$\mathrm{i}=\min(\zddtop(p),\zddtop(S))$}
\STATE {$p_0=\subsetzero(p,i)$}
\STATE {$p_1=\subsetone(p,i)$}
\STATE {$S_0=\subsetzero(S,i)$}
\STATE {$S_1=\subsetone(S,i)$}
\STATE {$Z_{00}=\zeros(p_0,S_0)$}
\STATE {$Z_{01}=\zeros(p_0,S_1)$}
\STATE {$Z_{11}=\zeros(p_1,S_1)$}
% Q.: Capital Z?
\RETURN $\zddite(i,S_1 \backslash (\symmdiff{Z_{01}}{Z_{11}}),Z_{00})$
% Ist S_1 \backslash (\symmdiff{Z_{01}}{Z_{11}} aufwendig?
% A:eher nicht
\end{algorithmic}
\end{algorithm}

Consequently, \algref{alg:recursive_ones} yields the remaining points.
%
\begin{algorithm}
% Rem.: ``|'' in textmode becomes something like --
\caption{Ones: $\ones(p,S)$}
\label{alg:recursive_ones}
\begin{algorithmic}
\REQUIRE Boolean polynomial $p$, $S$ set of points in $\Ztwo^n$ 
%represented as ZDDs
\ENSURE $\ones(p,S)=\{s\,|\,s \in S\;\text{and}\; p(s)=1\}$
\RETURN{$S\backslash \zeroes(p,S)$}
\end{algorithmic}
\end{algorithm}

%\subsection{Lexicographical normal form against ideals given as variety}
\subsection{Normal forms against a variety}

Normal forms are very hard to compute, 
in particular,  if \Groebner bases calculations are in use.
%
So, it is a quite natural question, whether the latter may be avoided by
introducing \specialised methods for calculating normal forms.
The presented method works even without a generating system of the ideal,
\ie in case it 
is just given in form of its variety.

Since ideals in the ring of Boolean polynomials are in one to one correspondence
to subset of~$\Ztwo^n$, this problem is quite general. 
Moreover, the \Groebner basis of the ideal can be a much bigger object than the corresponding variety.

\begin{defn}
Let $>$ be an arbitrary monomial ordering, then we can extend $>$ lexicographically to the set of Boolean polynomials (we make use of the fact, that there are no coefficients) by:
$p\geq q$ if and only if one of the following conditions holds.
% Rem.: Inconsistent notation \LEAD vs. lt (\lead?)
\begin{itemize}
\item $q=0$
\item $p\neq 0$, $q\neq 0$ and $\lm(p)>\lm(q)$
\item $p\neq 0$, $q\neq 0$, $\lm(p)=\lm(q)$ and $\tail(p)\geq \tail(q)$
\end{itemize}
\end{defn}


\begin{lemma}
\label{lemma:smallest_lex}
Let~$\fieldideal\subset I$ be an ideal, with~$I\subset \Ztwoxoneton$,
containing  a Boolean polynomial~$p$, and let~$G$ be a \Groebner basis of I.
Then the following two statements are equivalent:
\begin{enumerate}
\item $p$ is the lexicographical smallest Boolean polynomial in~$p+I$.
\item $\rednf(p,G)=p$ (\ie p is reduced).
\end{enumerate}
\end{lemma}

\begin{pf}
A Polynomial is reduced, if and only if all its terms are reduced (standard monomials).

So assume, that a term~$t$ of~$p$ is not reduced: Then there exists an~$f \in
G$, 
\sth~$t$ can be rewritten by~$f$  modulo~$I$. Applying the field equations the result is again a Boolean polynomial. 
In this way, we have constructed a smaller Boolean polynomial in~$p+I$.

On the other hand, let $p$ be reduced. Assume, there exists a smaller polynomial $q$ in the same residue class.
%
W.\,l.\,o.\,g.\ assume~$\lm(p)\neq \lm(q)$.
Then we know from general \Groebner basis theory, that $\rednf(p,G)=\rednf(q,G)$. Since $p$ is reduced, it follows $p=\rednf(q,G)$ and $p-q$ has a standard representation (each summand has a leading term smaller or equal to $\lm(p)=\lm(p-q)$).

Hence, it follows, that one of the summands in this presentation has $\lm(p)$
as leading term and $p$ is not reduced.
\end{pf}

In order to show the basic principles of interpolating with Boolean
polynomials, we provide a simple interpolation procedure given in
\algref{alg:interpolate_simple}.
%
\begin{algorithm}
\caption{$\interpolateSimple(b_Z^O)$}
\label{alg:interpolate_simple}
\begin{algorithmic}
\REQUIRE{$b_Z^O$ a partial function definition.}
\ENSURE$\interpolateSimple(b_Z^O)= p$, \sth~$f_p=b_Z^O$ on~$Z\cup O$
\IF{$Z = \emptyset$}
\RETURN $1$
\ENDIF
\IF{$O = \emptyset$}
\RETURN $0$
\ENDIF
\STATE {$i=\min(\zddtop(O),\zddtop(Z))$}
\STATE {$Z_1=\subsetone(Z,i)$}
\STATE {$Z_0=\subsetzero(Z,i)$}
\STATE {$O_1=\subsetone(O,i)$}
\STATE {$O_0=\subsetzero(O,i)$}

\STATE {$h_e=\interpolateSimple(b_{Z_0}^{O_0})$}
\STATE {$h_t=\interpolateSimple(b_{Z_1}^{O_1})+h_e$}
\RETURN {$x_{i}\cdot h_t+h_e$}
\end{algorithmic}
\end{algorithm}
%
If two sets~$Z$ and~$O$ of vectors are given, we can reduce the
interpolation problem to the case, where the $i$-th index of all vectors
is~$0$. For this purpose let~$Z_0, O_0$ denote the sets of those
vectors,  whose $i$-th entry is zero~(subset-0 points). Analogously,
for~$S\in\{Z,O\}$ let~% 
$S_1=\set{(v_1, \dots, v_{i-1}, 0,v_{i+1}, \dots v_n )  \,|\,  v\in S
\;\text{and}\; v_i=1 } $ denote the
subset-1 points.




First, we calculate  an interpolation~$h_e$ for the points~$Z_0 \cup 0_0$.
In the second step, we may continue with an interpolation~$h$ of the subset-1
points in~$Z_1 \cup 0_1$. 
%
One could combine both recursively generated results
to~$x_i \cdot h + h_e$, but this yields wrong results for vectors
in~$O_1\cap O_0$. This can easily be fixed, by \cancelling those terms already
treated by~$h_e$. In this case, it can be done just by adding~$h_e$ to~$h$,
because the terms with~$x_i$ do not influence the behaviour
on~$Z_0 \cup O_0$. 
For this reason $h_e$ is computed first.


On the other hand, if we really want to have a minimal interpolation polynomial, then we should not adjust the bigger terms (those with $x_i$: $x_i\cdot h_t$) to the smaller terms (those without $x_i$), but do the opposite.
So we would like to compute~$h_t$ first.
The problem is, if we want to calculate the then-branch of the interpolation
polynomial $h_t$, then we have to know the value $h_e$ takes on the
interpolation points specified for~$h_t$. Moreover, we should not specify more interpolation points than needed for~$h_t$, as for every point in~$Z_1 \cup O_1$, which does not lie in $Z_0 \cup O_0$ the value of the function can be adjusted by~$h_e$.
Luckily the behaviour of $h_e$ on $(Z_1 \cup O_1)\cap (Z_0 \cup O_0)$ is predictable and this gives exactly the set of interpolation points, which we will specify for $h_t$.
This approach is incorporated in \algref{alg:interpolate_smallest_lex}.
%
% Rem.: Lange Kommentare in die Erläuterung des Algorithmus.
\begin{algorithm}[htb]
\caption{$\interpolateSmallestLex(b_Z^O)$}
\label{alg:interpolate_smallest_lex}
\begin{algorithmic}
\REQUIRE{$b_Z^O$ a partial function definition.}
\ENSURE$\interpolateSmallestLex(b_Z^O)$, smallest Boolean
polynomial~$p$ \wrt lex.,  \sth~$f_p=b_Z^O$ on~$Z\cup O$

\IF{$Z = \emptyset$}
\RETURN $1$
\ENDIF
\IF{$O = \emptyset$}
\RETURN $0$
\ENDIF
% Rem.: Hm, bisher war top immer die Variable nicht der Index.
\STATE {$i=\min(\zddtop(O),\zddtop(Z))$}
% \subsetone(Z, index) usw. ???
%?????
\STATE {$Z_1=\subsetone(Z,i)$}
\STATE {$Z_0=\subsetzero(Z,i)$}
\STATE {$O_1=\subsetone(O,i)$}
\STATE {$O_0=\subsetzero(O,i)$}
\STATE {$C=(Z_1\cup O_1) \cap (Z_0\cup O_0)$}
\COMMENT {$C$ forms the set of conflict points between 0 and 1-subsets}

\STATE {$f=b_{Z_1}^{O_1}$}
\STATE {$g=b_{Z_0}^{O_0}$}

\STATE {$h_t=\interpolateSmallestLex(f+g)$}
\COMMENT {f+g is only defined on $C$}
\STATE {$F=\ones(h_t,((Z_1 \cup O_1)\backslash C))$}


\COMMENT {non-conflict subset1 terms affected by else branch}
% Rem.: Wieso sind \symmdiff{(Z_1 \backslash C)}{F} und (\symmdiff{(O_1
% \backslash C)}{F} disjunkt?
% Hm, ne klar. Was in F ist und vorher in O1 ist abgehakt und ``wandert'' durch
% die beiden symmdiff nach von O1 nach Z1. Umgekehrt für die neuen
% ``Einsstellen'' in F.
\STATE {$w=b_{(\symmdiff{(Z_1 \backslash C)}{F}) \cup Z_0}^{(\symmdiff{(O_1 \backslash C)}{F}) \cup O_0}$}

\STATE {$h_e=\interpolateSmallestLex(w)$}

\RETURN {$x_{i}\cdot h_t+h_e$}


\end{algorithmic}
\end{algorithm}
%
The following results show, that the algorithm computes the desired
interpolation.

%\begin{thm}
%    Algorithm \ref{alg:interpolate_smallest_lex} calculates the lexicographically smallest interpolation polynomial for the partial function specified.
%\end{thm}
%\begin{pf}
% 
%\end{pf}
% Rem.: Cofactor?
\begin{lemma}
	\label{lem:when_smallest}
Let $S$ be a set of non-constant Boolean polynomials, $v$ the smallest top variable occurring in
$S$ (biggest index: $\max\{\zddtop{f} \vert f \in S\}$), $S\owns p=v\cdot p_1+p_0$ ($v$ not occurring in $p_1$, $p_0$).
Then $f$ is lexicographically smallest polynomial w.\,r.\,t.\ lex.\ monomial
ordering if and only if~$p_1$ is the minimal cofactor in $S$ and for all $g\neq p$ with
$g=v\cdot p_1+g_0$ holds: $g_0>p_0$.
\end{lemma}
\begin{pf}
    This lemma is a consequence of the fact, that if~$p=v\cdot p_1+p_0$ with~$v$ as top variable, all terms, in which~$v$ occurs are bigger than those without~$v$, so are considered first in lexicographical comparison of Boolean polynomials.
\end{pf}
\begin{thm}
Algorithm \ref{alg:interpolate_smallest_lex} returns an interpolation polynomial, which is the lexicographically smallest polynomial w.\,r.\,t.\ lex.\ monomial ordering under all polynomials interpolating the same function on $P$.
\end{thm}

% Rem: Muss ich mir nochmal durchlesen, hab ich noch nicht bis in die Tiefe
% verstanden (AD).
\begin{pf}
We can assume, that all recursive calls deliver a polynomial with the desired property.

It can be checked easily, that the result provides an interpolation of the specified function by doing case considerations.

 To see, that it is minimal we use the previous lemma for minimality:
 First, we have to check, that $h_t$ is chosen minimal.
 By our assumptions the recursion returns a minimal polynomial under the specified properties.
 So, we know that it is minimal under all possible choices for the then-branch $h_t$ of our interpolation polynomial, \fulfil the specified condition (which means that the recursive call chooses the minimal polynomial out of the full set of candidates).
 So we just have to check, that all conditions are necessary for the then-branch of an interpolation polynomial.


 In fact we only prescribe the behaviour of $h_t$ on all conflicting points, such originally prescribed points, which occur in both combinations: with index $i$ set to $0$ one time (we denote that set in the following by $C_0$), and one time index $i$ set to $1$ ($C_1$).
 
 For this points we have the following situation: $$\forall c \in C_0: h_e(c)=h_e(c_{x_i=1}), c_{x_i=1}\in C_1, x_i \cdot h_t(c)=0$$
 So, no matter, what $h_t$ we choose, we get
 $$h_e(c)=1\Leftrightarrow c \in O_0 \;\text{for all}\; c \in C_0.$$
 So, we conclude:
%
\begin{eqnarray*}
\forall c \in C_1: h_t(c)=1\Leftrightarrow (c \in O_1 \text{ and } c_{x_i=0} \in
Z_0) \text{ or }\\ (c \in O_0 \text{ and } c_{x_i=0} \in Z_1)
\end{eqnarray*}
 This conditions on $h_t$ are equivalent to the partial Boolean function definition $f+g$.
 So the specification $f+g$ for our then-branch contains only necessary interpolation points and recursively we get a minimal interpolation polynomial for this part.
 So we fulfilled the first condition of our lemma and calculated a minimal $h_t$ under all interpolation polynomials.
 Note, that if the index $i$ we branch at, is not biggest possible for an interpolation $h_t$ will be just zero, so that is also compatible with the lemma.

 Having the correct $h_t$, we have to check, that under all Boolean interpolation polynomial of the form $x_i \cdot h_t + h_e$, we choose a minimal $h_e$. The behaviour as function of $h_e$ is uniquely determined on $Z \cup O$ by $h_t$ and the prescribed interpolation values, and this is just, what our recursive call for calculating $h_e$ does: passing these (possibly adjusted) values.
 Since all candidates for $h_e$ needs to \fulfil this condition, we really get the full sets of candidates and by recursion a minimal else branch.
\end{pf}

\begin{lemma}
	For each monomial ordering $>$ and each set of points~$P$ the set of standard monomials $S$ \wrt~$I(P)$ in~$\Ztwoxoneton$ has the same cardinality as $P$:$$\vert S\vert=\vert P\vert\,\mbox{.}$$
\end{lemma}

\begin{pf}
$\set{s+I(P)|s \in S}$ is a basis of $\Ztwoxoneton/I(P)$ as a vector space,
and~$I(P)$ contains $\fieldideal$. $\Ztwoxoneton/\fieldideal$ has dimension
$2^n$ as a~$\Ztwo$-vector-space, which are in one to one correspondence to Boolean
functions. All Boolean polynomials from~$I(P)$ uniquely represent a Boolean
function, which is zero on~$P$. So~$I(P)$ contains~$2^{2^n-P}$ elements. It
follows, that the dimension of the quotient space
$$(\Ztwoxoneton/\fieldideal)/I(P)$$ is $\vert P \vert$. Furthermore, it equals
to the size of~$S$ as well, as it forms a basis.
% P z.T. als Zahl verwendet, \vert P\vert? (siehe auch nächstes Korollar)
\end{pf}

\begin{corollary}
Let $f\in \Ztwoxoneton$ be a Boolean polynomial, $P$ a set of points in~$\Ztwo^n$. Then a reduced normal form~$g=\rednf(f,I(P))$ has at most~$\vert P\vert$ terms.
\end{corollary}

\begin{algorithm}[htb]
\caption{Reduced lexicographical normal form against a variety: $\nfByInterpolate(f,P)$}
\label{alg:normal_form_variety}
\begin{algorithmic}
\REQUIRE Boolean polynomial $f$, P set of points in $\Ztwo^n$.
\ENSURE $\nfByInterpolate(f,P)=\NF(f,I(P))$
\STATE $Z=\zeros(f,P)$
\RETURN $\interpolateSmallestLex(b_Z^{P \backslash Z})$
\end{algorithmic}
\end{algorithm}
\begin{thm}
Algorithm \ref{alg:normal_form_variety} calculates a lexicographical normal form
of f against a \Groebner basis of the ideal $I(P)=\set{g \in \Ztwoxoneton|
g(p)=0 \;\text{for all}\; p \in P}$.
\end{thm}
\begin{pf}
First note: A reduced normal form against a \Groebner Basis $G$ does not depend on the particular choice of $G$, but only on the ideal generated by $G$.
Moreover, since Boolean polynomials are in one to one correspondence to Boolean functions, 
every Boolean polynomial representing the same function on $P$, lies in the same residue class modulo~$I(P)$.
A normal form $g=\NF(f,G)$ of a polynomial against a \Groebner basis $G$ can be
characterized, to be the unique reduced polynomial, since~$g=\NF(g,G)$, where~%
$g+\ideal{G}=f+\ideal{G}$.
So we have to show for given~$f$, and~$P$:
%
\begin{enumerate}
% Alg. nicht als \nfByInterpolate benannt
\item $\nfByInterpolate(f,P)$ represents the same function restricted to $P$ as $f$.
\item $\nfByInterpolate(f,P)$ is reduced.
\end{enumerate}
The first claim holds by the correctness, as we have already proven, that $\nfByInterpolate$ returns indeed an interpolating function.
The reducedness follows from Lemma \ref{lemma:smallest_lex}.
\end{pf}

\begin{algorithm}[htb]
\caption{Standard monomials of $I(P)$: \newline  $\standardMonomialVariety(P)$}
\label{alg:standard_monomials_variety}
\begin{algorithmic}
\REQUIRE P a set of points in $\Ztwo^n$.
% Rem.: Kann man das so sagen?
\ENSURE $S =
 \set{t \,|\,\exists \;\text{reduced}\;p \in I(P) : t \;\text{term of}\;p}$
\STATE $S=\emptyset$
\WHILE{$\vert P\vert\neq\vert S\vert$}
\STATE $Z=\randomSubset(P)$
\STATE $p=\interpolateSmallestLex(b_Z^{P \backslash Z})$
\STATE $S=\set{t \;\mbox{term}\;| \exists s \in S: t\vert s}$
\STATE $S=S\cup \support(p)$

\ENDWHILE
\RETURN $S$
\end{algorithmic}
\end{algorithm}

\begin{algorithm}[htb]
\caption{Leading monomials of a minimal \Groebner basis of $I(P)$}
\label{alg:leading_monomials}
\begin{algorithmic}
\REQUIRE P set of points in $\Ztwo^n$.
\ENSURE{$\leadingMonomialsVariety(P)=\LI(\I(P))$}
\STATE{$T=\set{t \mbox{ Boolean term in }\Ztwoxoneton}$}
\STATE $R=T\backslash \standardMonomialVariety(P)$
\RETURN{$\minimalElements(R)$}
\end{algorithmic}
\end{algorithm}


\begin{thm}
	Assume that the probability distribution of the choice of random subsets $Z$ are independent equipartitions for each point $p \in P$ and form independent experiments.
	Then the probability $p$ for the main loop of Algorithm~\ref{alg:standard_monomials_variety} passing more than $k$ iterations is~$1-(1-\frac{1}{2^k})^{|P|}$.
\end{thm}
\begin{pf}
    For a random subset $Z\subset P$, the probability, that a standard monomial $t$ occurs in the interpolation is $\frac{1}{2}$.
    The probability, that a term $t$ does not occur in $k$ experiments is $\frac{1}{2^k}$.
    Since the probability distribution of independent equipartitions  on $P$ result in independence on the set of standard monomials,
    the probability, that all $|P|$ standard monomial occur in $k$ experiments is~%
$\displaystyle(1-\frac{1}{2^k})^{|P|}$.
\end{pf}
%Interessantes Ergebnis!
% Rem.: Da sollte aber was zum Beweis stehen.

%\begin{remark}

All presented set operations~-- except the~$\randomSubset$ procedure~-- 
have been implemented in
a decision diagram-style recursive approach.
In particular, there is no problem to represent the set of terms $T$ with $2^n$ elements in it, as the number of ZDD-nodes is just~$n$ (in this case).
%
\begin{algorithm}
\caption{Reduced lex.\ \Groebner basis of $I(P)$}
\label{alg:points_gb}
\begin{algorithmic}
\REQUIRE $P$ set of points in $\Ztwo^n$.
% Rem.: Schau mal, ob das so gemeint war:
\RETURN{$\set{t+\nfByInterpolate(t, P)\,|\,t \in \LI(I(P))}$}
\end{algorithmic}
\end{algorithm}
%
%\end{remark}
%
\Algref{alg:points_gb} shows, that it is even possible to compute the complete \Groebner basis of $I(P)$ just having this normal form algorithm.
Of course the real value of this section is however to be able to compute these normal forms without computing the \Groebner basis.

\subsection{Practical experiments}
In this section we consider randomly generated examples and show, that we can still compute lexicographical normal forms, where the computation of the full \Groebner basis seems to be practically unfeasible.
These generating systems are usually quite big. In fact for \tabref{tab:InterpolVsGroebner} with our experiments, the size of the \Groebner basis was computed by the function~$\leadingMonomialsVariety$ returning the leading ideal. This is much cheaper than computing the \Groebner basis itself (at least using \algref{alg:points_gb} as you can see in the following). If you consider the size of the \Groebner basis $s$, the number of points $\vert P\vert$, the cost of a single normal form $N$. Then cost of computing the leading ideal is approximately $\log(\vert P\vert) \cdot N$ and for the \Groebner basis $s\cdot N$ (if you like, you can assume, that $s$ is in the same dimension as $\vert P\vert$). This is of course no exact complexity analysis, but gives some feeling for the problem.
For computing the normal form against the variety,  neither the \Groebner basis
is needed, nor the leading ideal, but just a single call
of~$\nfByInterpolate$. This is much easier, in particular because the \Groebner basis in the biggest example in this listing has about~$600000$ elements.
Due to the random nature of our examples, we expect the $\tail$ of each basis elements quite dense in the set of standard monomials, which has size $|P|$, $500000$ in this example.

Our timings have been done on a AMD Dual Opteron 2.2 GHz (we have used only one CPU) with 16 GB RAM on Linux.
We used random sets of points and random partial functions in 100 variables. Note, that random data is supposed to be the worst case scenario for \PolyBoRi, as using caching techniques our algorithms work better on structured polynomials.

We were not able to run $\interpolateSimple$ on the bigger example, since the memory consumptions was to high. On the other hand this algorithm shows nice performance to simplicity in the small examples (mainly, as the expensive call to $\zeros$ is missing).
In this sense, these results underline the picture, that our algorithm is able to compute normal forms without \Groebner basis up to a magnitude, in which is seems impossible to compute the \Groebner basis on nowadays machines in reasonable time.


\begin{table}
\begin{center}
\begin{tabular}{@{}r|rr|r@{}r|r@{}}
\multicolumn{1}{@{}c|}{\#} 
&\multicolumn{2}{c|}{smallest lex.}&\multicolumn{2}{c|}{$\interpolateSimple$}
&\multicolumn{1}{c@{}}{\#} \\
\multicolumn{1}{@{}c|}{points}
 &\multicolumn{2}{c|}{time/1\,s \hfill length}
 &\multicolumn{2}{c|}{time/1\,s \hfill length}
&\multicolumn{1}{c@{}}{basis}\\
\hline
$100$&$0.01$&$42$&$0.00$&$12771$&$287$\\
$500$&$0.06$&$249$&$0.01$&$\approx\!2.9\cdot 10^{10}$ %  28718707949  
  &$1943$\\
$1000$&$0.29$&$508$&$0.01$&$\approx\! 8.1\cdot 10^{13}$&$3393$\\
$5000$&$5.53$&$2552$&$1.47$&$\approx\! 4.5\cdot 10^{23}$&$10319$\\
$10000$&$19.78$&$5020$&$37.18$&$\approx\!1.6\cdot 10^{26}$&$17868$\\
$50000$&$250.95$&$25012$&&&$82929$\\
$100000$&$897.85$&$50093$&&&$162024$\\
$200000$&$3488.61$&$99868$&&&$296697$\\
$500000$&$20336.02$&$249675$&&&$636542$\\
\end{tabular}
\caption{Interpolation vs.\ \Groebner approaches.}
\label{tab:InterpolVsGroebner}
\end{center}
\end{table}

==> lp.tex <==
\tablefirsthead{Example & \multicolumn{2}{c|}{Vars./Eqs.}
  & \multicolumn{2}{c}{\PolyBoRi} &
  \multicolumn{2}{c}{\Singular}& \multicolumn{2}{c}{\Magma}& 
  \multicolumn{2}{c}{Maple}\\ \hline}

\tablehead{Example & \multicolumn{2}{c|}{Vars./Eqs.}
  & \multicolumn{2}{c}{\PolyBoRi} &
  \multicolumn{2}{c}{\Singular}& \multicolumn{2}{c}{\Magma}& 
  \multicolumn{2}{c}{Maple}\\ \hline}

\tabletail{\hline}
\tablelasttail{\hline}

\newcommand{\niceGreater}{\ensuremath{\!\!>\!\!}}
%
\begin{mpsupertabular}{lrr|rrrrrrrr}
\label{weighted lengths}
ctc-5-3   &   189    & 354 &$3.04$\,s     &      49\,MB         & 32\,s& 69\,MB& $83$\,s & $64$\,MB &$\niceGreater{}1800$\,s&$\niceGreater{}89$\,MB\\
ctc-8-3   &    297   & 561     &  $4.8$\,s   &     52\,MB      & 117\,s& 154\,MB&817s & 335\,MB&&\\
ctc-15-3   &   549    &  1044 &  $8.04$\,s   &     69\,MB      &748\,s & 379\,MB & $\niceGreater{}3000$\,s & $\niceGreater{}570$\,MB&&\\
aes-10-1-1-4pp   &   164    &  184    &    $0.14$\,s  &  $^\textrm{\ref{fn:toofast}}$         & $0.25$\,s &   &    $0.92$\,s     &    $9.25$\,MB     & $\niceGreater{}1000$\,s & \\
aes-7-1-2-4pp    & 204      & 255     &    $3.24$\,s  &   50\,MB        &  $18$\,s&    &       366s     &  211\,MB         &          &    \\
aes-10-1-2-4pp&  288  &  318 &   6.7\,s     &    51\,MB   &  1080\,s    &   694\,MB  &   1007\,s &  476\,MB  & $\niceGreater{}70$\,h & $\niceGreater{}324$\,MB\\
mult4x4       &55     &48    &  0.01\,s     & \footnote{\label{fn:toofast}too short to trace memory usage}        &0.01\,s    &0.7\,MB     &   0.91\,s &  10\,MB &  0.99\,s  & 9.8\,MB    \\
mult5x5       &  83   & 84   &  0.022\,s    &  $^\textrm{\ref{fn:toofast}}$     & 0.03\,s     &0.7\,MB    &    31.5\,s & 44\,MB  &    23.89s& 16\,MB       \\
mult6x6       &  117  & 106  &  0.047\,s    &  $^\textrm{\ref{fn:toofast}}$      & 0.169\,s     &2.9\,MB    &   4582\,s  &  1044\,MB &        &        \\
mult8x8       &  203  &188   &  1\,s        &  $^\textrm{\ref{fn:toofast}}$    &  106\,s     &   153\,MB  &           &       &        &        \\   
mult10x10     &313    &294   &  2.5\,min    &  86\,MB    &           &          &           &       &        &        \\    
\end{mpsupertabular}
\tabletail{}
\tablelasttail{}
\tablehead{}
\tablefirsthead{}


==> modulomonomials.tex <==
% Rem.: Hab den Abschnitt mal zur \subsection degradiert, da er sonst etwas in
% der Luft haengt. 
\subsection{Normal form against a set of monomials}

In this section we give a first, easy example of ZDD-style recursive normal form computations for special systems of generators.
Consider a Boolean polynomial $f$ and a set of (Boolean) monomials $G$.
Then we have $g=\rednf(f,G)$ if and only if~$g \in f+\ideal{G}$.
Note, that it does not matter in this case, if we add the field polynomials to $G$.

We can identify the set~$G$ with a polynomial, where exactly the elements of~$G$ appear with coefficient~$1$.
So, both~$f$ and~$G$ can be represented as ZDDs.
%
Hence, we will formulate the procedure recursively in the language of ZDDs,
but for the sake of simplicity, we skip
caching in the pseudo-code.%leave out anything, which has to do
                               %with caching. 

Computing the normal form of a polynomial $f$ against a set of monomials $G$, means just \cancelling all terms in $f$, which are divisible by an element of $G$.
\Algref{alg:modulomonomials} does it very efficiently (properly implemented) and it is the easiest example for directly computing the reduced normal form recursively without the classical Buchberger normal form algorithm.
%
\begin{algorithm}
\caption{Normal form against a set of monomials}
\label{alg:modulomonomials}
\begin{algorithmic}
\REQUIRE $f$ a polynomial, $G$ a set of monomials, both encoded as ZDD.
\ENSURE $\nfMonSet(f, G) =\rednf(f,G)$
\IF {$1 \in G$}
\RETURN{$0$}
\ENDIF
%\IF{ $G==\emptyset$}
%\RETURN{f}
%\ENDIF

\IF{$f\in\set{0, 1}$}
\RETURN{$f$}
\ENDIF
\WHILE{$\zddtop(f)>\zddtop(G)$}%!!!! index: important for the > sign
\STATE{$G=\elseBranch(G)$}
\ENDWHILE


\IF{ $G=\emptyset$}
\RETURN{f}
\ENDIF
\COMMENT{monomial in which $\zddtop(f)$ occurs must be tested for divisibility with the then and the else-branch of $G$}
\IF{$\zddtop(f)=\zddtop(G)$}

\RETURN{$\ite(\zddtop(f),$\\\quad$\nfMonSet(\nfMonSet(\thenBranch(f),\elseBranch(G)),\thenBranch(G)),$\\\quad$\nfMonSet(\elseBranch(f),\elseBranch(G)))$}
\ELSE
\RETURN{$\ite(\zddtop(f),\nfMonSet(\thenBranch(f),G),$\\\quad$\nfMonSet(\elseBranch(f),G))$}
\ENDIF
\end{algorithmic}
\end{algorithm}


==> pbresults-aug07.tex <==
\section{Timings}
\providecommand{\secunit}{\ensuremath{\,\mathrm{s}}}
\providecommand{\MBunit}{\ensuremath{\,\mathrm{MB}}}

\providecommand{\timedoutAfter}[1]{\multicolumn{1}{c}{$\infty$} & }
\providecommand{\memoryout}{ &\,\hfill$\infty$\hfill\, }
% Alternative, explicitely stating time/memory excess
%\renewcommand{\timedoutAfter}[1]{\multicolumn{1}{c}{$>$#1}&}
%\renewcommand{\memoryout}{&\,\hfill$>15\,\mathrm{GB}$\hfill\, }
\providecommand{\timedout}{\timedoutAfter{1\,h}}
\providecommand{\Singular}{{\sc Singular}}
\providecommand{\Magma}{{\sc Magma}}
\providecommand{\PolyBoRi}{{\sc PolyBoRi}\xspace}
\providecommand{\symmgbGFTwo}{symmgbGF2\xspace}
\providecommand{\Groebner}{Gr\"{o}bner\xspace}
\providecommand{\behaviour}{behaviour\xspace}
\providecommand{\optimis}{optimis}
\providecommand{\optimised}{\optimis{}ed\xspace}
\providecommand{\optimise}{\optimis{}e\xspace}
\providecommand{\optimisation}{\optimis{}ation\xspace}
\providecommand{\optimisations}{\optimisation{}s\xspace}
\providecommand{\specialised}{specialised\xspace}
\providecommand{\modell}{modell}
\providecommand{\practise}{practise\xspace}
\providecommand{\summarised}{summarised\xspace}
\providecommand{\minimise}{minimise\xspace}
\providecommand{\utilise}{utilise\xspace}
\providecommand{\utilises}{utilises\xspace}
\providecommand{\utilised}{utilised\xspace}
\providecommand{\utilisation}{utilisation\xspace}
\providecommand{\utilising}{utilising\xspace}
\providecommand{\homogenisation}{homogenisation\xspace}
\providecommand{\generalisation}{generalisation\xspace}
\providecommand{\analys}{analys}
\providecommand{\emphasise}{emphasise\xspace}
\providecommand{\tabref}[1]{Table~\ref{#1}}
\providecommand{\Tabref}[1]{Table~\ref{#1}}
\providecommand{\citep}{\cite}
\providecommand{\citetext}[1]{[#1]\xspace}
\providecommand{\ie}{i.\,e.\xspace}
\providecommand{\eg}{e.\,g.\xspace}


This section presents some benchmarks comparing \PolyBoRi to general purpose and
\specialised computer algebra systems.
%
The following timings have been done on a AMD Dual Opteron 2.2 GHz (all systems
have used only one CPU) with 16 GB RAM on Linux.
%
The used ordering was lexicographical, with the exception of FGb, where
degree-reverse-lexicographic was used.
\PolyBoRi also implements degree
orderings, but for the presented practical examples elimination orderings seem to
be more appropriate. A recent development in \PolyBoRi was the implementation of
block orderings, which behave very natural for many examples.


We compared the following system releases with the development version
of \PolyBoRi's \symmgbGFTwo:

\begin{tabular}{lll}
Maple& 11.01, June 2007 & Gr\"obner package, default options\\
FGb &  1.34, Oct.\ 2006 &  via Maple 11.01, command: fgb\_gbasis\\
\Magma & 2.13-10, Feb.\ 2007&  command: GroebnerBasis, default options\\
\Singular& 3-0-3, May 2007 & std, option(redTail)\\% (= \PolyBoRi's default) 
\end{tabular}

 Note, that this  presents the state of
\PolyBoRi in the development version  in August 2007 only. Since the
project is still very young there is still room for major performance
improvements.

The examples were chosen from current research problems in formal verification
and algebraic crypto analysis.
The latter yields systems of equations, which are comparable to those arising
from formal verification, but they are more scalable.
%
We use an algebraic attack to a small scale variant of the
\emph{Advanced Encryption Standard}~(AES)~\citep{FIPS197}.
This approach is based on~\cite{CidMurRob05} and
was provided by Stanislav Bulygin~\citetext{private communication}.  We made
some \optimisations on the
formulation of the equations in the formulation.
Furthermore,  examples using \emph{Courtois Toy Cipher}~(CTC),
which are due to Martin Albrecht~\citep{AlbrechtM}, were tested.
The systems describing the formal verification of
multipliers were provided by Markus Wedler~\citetext{private communication}.

All timings of the computations are \summarised in \tabref{table:results}.
%
% Status: 2007-08-20, 2007-08-28 (fgb + PolyBoRi memory peak)
\begin{table}
\begin{center}
{\tiny
\newcommand{\cstyle}{{\hspace{.6em}}}
\renewcommand{\MBunit}{}
\renewcommand{\secunit}{}
\begin{tabular}{crr|rr||@{\cstyle}r@{\cstyle}r@{\cstyle}|@{\cstyle}r@{\cstyle}r@{\cstyle}|@{\cstyle}r@{\cstyle}r@{\cstyle}|@{\cstyle}r@{\cstyle}r@{\cstyle}}
\multicolumn{3}{c}{} & \multicolumn{2}{c}{\PolyBoRi} & 
  \multicolumn{2}{c}{FGb}&
  \multicolumn{2}{c}{Maple}&
  \multicolumn{2}{c}{\Magma} & \multicolumn{2}{c}{\Singular}
\\
Example &\multicolumn{2}{@{\cstyle}c|}{Vars./Eqs.} &

\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c||@{\cstyle}}{MB} &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c|@{\cstyle}}{MB} &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c|@{\cstyle}}{MB} &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c|@{\cstyle}}{MB}  &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c}{MB}

\\
\hline
aes\_7\_1\_2\_4\_pp&  204 &  225  &
0.15\secunit & 53.82\MBunit
& % Format: fgb
2812.30\secunit & 10.12\MBunit
 & %Format : maple
\timedout %0.70\secunit &  11.00\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
346.37\secunit & 206.22\MBunit
 & %Format : sing
27.41\secunit & 25.77\MBunit
\\
aes\_10\_1\_1\_4\_pp&  164 &  184  &
0.02\secunit & 52.70\MBunit
& % Format: fgb
1.97\secunit & 9.37\MBunit
 & %Format : maple
2.99\secunit & 10.37\MBunit
 & %Format : magma
0.87\secunit & 9.03\MBunit
 & %Format : sing
0.02\secunit& 1.75\MBunit
\\
aes\_10\_1\_2\_4\_pp&  288 &  318  &
0.22\secunit & 55.59\MBunit
& % Format: fgb
\timedout %Error:1.960\secunit & 10.37\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %1.36\secunit & 12.50\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
847.91\secunit & 471.58\MBunit
 & %Format : sing
183.73\secunit & 55.86\MBunit
\\


ctc\_3\_3&  117 &  117  &
0.04\secunit & 52.80\MBunit
& % Format: fgb
6.56\secunit & 8.62\MBunit
 & %Format : maple
10.40\secunit &  10.37\MBunit
 & %Format : magma
1.62\secunit & 10.39\MBunit
 & %Format : sing
0.77\secunit & 5.25\MBunit
\\
ctc\_5\_3&  189 &  189  &
0.10\secunit & 63.05\MBunit
& % Format: fgb
602.20\secunit & 9.75\MBunit
 & %Format : maple
929.77\secunit & 10.87\MBunit
 & %Format : magma
85.20\secunit & 67.79\MBunit
 & %Format : sing
3.63\secunit & 14.75\MBunit
\\
ctc\_8\_3&  297 &  297  &
0.15\secunit & 64.23\MBunit
& % Format: fgb
\timedout%Error:0.920\secunit & 9.87\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %0.86\secunit & 12.50\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
759.51\secunit & 299.08\MBunit
 & %Format : sing
14.32\secunit & 33.31\MBunit
% End of sing
\\
ctc\_15\_3&  549 &  549  &
0.28\secunit & 68.71\MBunit
& % Format: fgb
\timedout%Error:3.020\secunit & 11.25\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %2.67\secunit &  17.12\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
\timedout
 & %Format : sing
66.63\secunit & 116.98\MBunit
\\
\hline
mult3x3&  33 &  28  &
0.01\secunit & 54.52\MBunit
& % Format: fgb
0.07\secunit & 3.50\MBunit
 & %Format : maple
0.04\secunit & 3.00\MBunit
 & %Format : magma
0.57\secunit & 6.55\MBunit
 & %Format : sing
0.01\secunit & 0.64\MBunit
\\
mult4x4&  55 &  48  &

 0.00\secunit & 54.54\MBunit
& % Format: fgb
1.76\secunit & 5.50\MBunit
 & %Format : maple
1.96\secunit & 4.87\MBunit
 & %Format : magma
0.91\secunit & 10.48\MBunit
 & %Format : sing
0.02\secunit & 0.66\MBunit
\\
mult5x5&  83 &  74  &

 0.01\secunit & 54.66\MBunit
& % Format: fgb
219.09\secunit & 6.37\MBunit
 & %Format : maple
236.14\secunit &  6.87\MBunit
 & %Format : magma
31.28\secunit & 46.05\MBunit
 & %Format : sing
0.01\secunit & 1.67\MBunit
\\
mult6x6&  117 &  106  &
0.03\secunit & 54.92\MBunit
& % Format: fgb
\multicolumn{2}{c|@{\cstyle}}{failed}%
%bytes used=17585984, alloc=9304408, time=0.28
%Error, (in FGb:-fgb_gbasis) Limite de to_do est a 348406 !
 & %Format : maple
\timedout %3586.97\secunit & 1148.16\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
\timedout
 & %Format : sing
4.28\secunit & 21.19\MBunit
\\
mult8x8&  203 &  188  &

0.40\secunit & 55.43\MBunit
& % Format: fgb
\timedout%Error:3.210\secunit & 63.36\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %2.93\secunit & 50.99\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
\timedout
 & %Format : sing
\memoryout   %2.17\secunit & error: no more memory bytes
\\
mult10x10&  313 &  294  &

 18.11\secunit & 85.91\MBunit
& % Format: fgb
\memoryout
 & %Format : maple
\memoryout & %Execution Stopped: Memory allocation failed
 %Format : magma
\memoryout & %Format : sing
\memoryout %220.37\secunit & error: no more memory bytes
\end{tabular}
}
\end{center}
\caption{Timings and memory usage for benchmark examples. The infinity symbols
in time and memory columns
mark timeout after one hour and out of memory, respectively.}
\label{table:results}
\end{table}
%
The first part of table was computed with the help of \optimised routines.
It preprocess the equations in the 
following way: first auxiliary variables are eliminated, 
then a logical conjugation of the system is generated using  Boolean 
multiplication, which gives the unique Boolean ideal generator.%
%(see \thmref{unique-generator}).


The authors of this article are quite convinced, that the default strategy of
\Magma\ is not well suited for these examples (walk, see \cite{CoKaMa97}, or
\homogenisation). However, when we tried a direct approach in \Magma, it ran
very fast out of memory~(at least in the larger examples). So we can conclude,
that the implemented \Groebner basis algorithm in \PolyBoRi offers a good
performance combined with suitable memory consumption.
Part of the strength in directly computing \Groebner bases (without walk or
similar techniques) is inherited from the slimgb algorithm in \Singular.  On the
other hand our data structures provide a fast way to rewrite polynomials, which
might be of bigger importance than sparse strategies in the presented examples.

%While we used the normal slimgb algorithm for the presented examples, we were
%able to tackle much harder problems like 12BIT-Multiplier, AES small scale
%chiffre SR(10-1-2-8), SR(10-2-1-8), SR(10-2-2-4) using \optimised scripts.


In order to treat classes of examples, for which the lexicographical ordering is
not the best choice, \PolyBoRi is also equipped with other monomial orderings. 
Although, its internal data structure is ordered lexicographically, 
the computational overhead of the degree orderings implementation is small
enough, that the advantage of these orderings become effect.
%
\Tabref{tab:orderbench} illustrates this for a series of random unsatisfiable
examples~\cite{satlib00}. The latter arise from benchmarking SAT-solvers, which can handle them
very quickly, as their conditions are easy to contradict. But they are still a
challenge for the algebraic approach.
%
\begin{table}
\begin{center}
{\tiny
\begin{tabular}{cccc|rr||rr|rr}
 % \multicolumn{4}{c}{} & 
 % \multicolumn{2}{c}{\PolyBoRi} &
 % \multicolumn{2}{c}{\Magma} & 
 % \multicolumn{2}{c}{FGb} 
\\
Example &\multicolumn{2}{c}{Vars./Eqs.} & Order. &

  \multicolumn{2}{c||}{\PolyBoRi} &
  \multicolumn{2}{c|}{\Magma} & 
  \multicolumn{2}{c}{FGb} 

%\multicolumn{1}{c}{s} & \multicolumn{1}{c||}{MB} &
%\multicolumn{1}{c}{s} & \multicolumn{1}{c|}{MB}  &
%\multicolumn{1}{c}{s} & \multicolumn{1}{c}{MB} 
\\
\hline
uuf50\_8&  50 &  218  &
lp &
11.58\secunit & 71.58\MBunit
 & %Format : magma
12.88\secunit & 26.04\MBunit
   \\
&&& dlex&
10.95\secunit & 71.06\MBunit
 & %Format : magma
13.45\secunit & 29.02\MBunit
   \\
&&&dp\_asc&
7.78\secunit & 70.82\MBunit
 & %Format : magma
9.83\secunit & 37.02\MBunit
 & %Format : FGb
76.27\secunit & 6.75\MBunit
\\
%lp
uuf50\_9&  50 &  218  &
lp&
8.48\secunit & 71.12\MBunit
 & %Format : magma
14.82\secunit & 34.68\MBunit
   \\
&&&dlex&
10.15\secunit & 71.36\MBunit
 & %Format : magma
13.37\secunit & 36.45\MBunit
    \\
&&&dp\_asc &
14.11\secunit & 74.77\MBunit
 & %Format : magma
13.12\secunit & 33.06\MBunit
 & %Format : FGb
92.53\secunit & 6.75\MBunit
\\
uuf50\_10&  50 &  218  &
lp &
8.76\secunit & 71.98\MBunit
 & %Format : magma
9.77\secunit & 28.21\MBunit
   \\
&&& dlex&
8.98\secunit & 72.53\MBunit
 & %Format : magma
10.35\secunit & 32.71\MBunit
   \\
 &&& dp\_asc&
8.14\secunit & 72.24\MBunit
 & %Format : magma
8.40\secunit & 27.42\MBunit
 & %Format : GFb
74.76\secunit & 6.75\MBunit
\\
uuf75\_8&  75 &  325  &
lp &
843.38\secunit & 819.80\MBunit
 & %Format : magma
14015.21\secunit & 1633.62\MBunit
   \\
&&& dlex &
553.43\secunit & 490.86\MBunit 
 & %Format : magma
14291.45\secunit & 2439.53\MBunit
   \\
 &&& dp\_asc&
448.53\secunit & 472.04\MBunit 
 &  %Format : magma
13679.42\secunit & 2539.24\MBunit
& % Format: FGb
99721.46\secunit    & 8958.36\MBunit% \timedoutAfter{24\,h}
\\
uuf100\_01&  100 &  430  &
lp &
44779.77\secunit & 12309.79\MBunit
 & %Format : magma
 \timedoutAfter{2\,days}
\\
  &&&dlex &
11961.86\secunit & 6101.43\MBunit
& %Format : magma
 \timedoutAfter{2\,days}
\\
&&&dp\_asc &
10635.72\secunit & 6146.47\MBunit 
 & %Format : magma
\timedoutAfter{2\,days} 
& % Format: FGb
\multicolumn{2}{c}{failed}
% at sculptor, 2.4GHz alloc=9959648, time=57135.11
%Error, (in FGb:-fgb_gbasis) Limit for allocations (1-->1000): in
%update_all_garbages !
\end{tabular}
}
\end{center}
\caption{Timings and memory usage for benchmark examples, w.\,r.\,t.\ various
orderings. 
The infinity symbols mark timeout after two days.
%The infinity symbols in time and memory columns
%mark timeout after one day and out of memory, respectively.
}
\label{tab:orderbench}
\end{table}
%
The strength of \PolyBoRi is visible in the more complex examples, as it scales
better than the other systems in tests.

In addition the performance of \PolyBoRi is compared  with the freely
available SAT-solver MiniSat2~(release date 2007-07-21),  which is
state-of-the-art
among publicly available solvers~\citep{een03minisat}.
The examples consist of formal verification
examples corresponding to digital circuits with $n$-bitted multipliers
and the pigeon hole benchmark, which is the most important
standard benchmark problem for
SAT-solvers, \eg used in in~\cite{satlib00}, and some small-scale AES examples
again.
The latter checks whether it is possible to place~$n+1$ pigeons in~$n$ holes
without two of them being in the same hole~(obviously, it is unsatisfiable).

%minisat2 2007-07-21
%
\begin{table}
\begin{center}
{\scriptsize
\begin{tabular}{l|rr|rr|rr}
& \multicolumn{2}{c|}{Vars./Eqs.}  &
    \multicolumn{2}{c|}{\PolyBoRi}  &  \multicolumn{2}{c}{MiniSat}  \\
\hline
 hole6 & 42 & 133 &
 0.13\secunit & 51.64\MBunit &
 0.01\secunit & 1.96\MBunit \\
 hole7 & 56 & 204 &
 0.46\secunit & 51.89\MBunit &
 0.06\secunit & 1.96\MBunit \\
 hole8 & 72 & 297 &
 1.88\secunit &56.59\MBunit &
 0.30\secunit & 2.08\MBunit \\
 hole9 & 90 & 415 &
 8.01\secunit & 84.04\MBunit &
 2.31\secunit & 2.35\MBunit \\
 hole10 & 110 & 561 &
 44.40\secunit & 97.68\MBunit &
 25.20\secunit & 3.24\MBunit \\
% hole 11 & 12 added 2007-31-10
 hole11 & 132 &738  &
 643.14\secunit & 130.83\MBunit &
 782.65\secunit & 7.19\MBunit  \\ 
 hole12 & 156 &949   & 
  10264.92\secunit & 338.66\MBunit & 
  22920.20\secunit & 17.13\MBunit  
aes\_2\_2\_2\_4&  128 &  128  &
 3.93\secunit & 64.91\MBunit &
 12.04\secunit & 4.73\MBunit
\\
aes\_3\_2\_2\_4&  184 &  184  &
 46.67\secunit & 88.77\MBunit &
 76.88\secunit & 6.77\MBunit
\\
aes\_10\_1\_1\_8&  328 &  328  &
 2.26\secunit & 132.74\MBunit &
 58.30\secunit & 38.13\MBunit
\\
aes\_10\_2\_2\_4&  576 &  576  &
 1193.19\secunit & 150.70\MBunit &
 190.58\secunit & 15.03\MBunit
\\
aes\_7\_1\_2\_4\_pp&  204 &  225  &
 0.15\secunit & 53.82\MBunit &
 0.38\secunit & 5.16\MBunit
\\
aes\_10\_1\_1\_4\_pp&  164 &  184  &
 0.02\secunit & 52.70\MBunit &
 0.03\secunit & 3.49\MBunit
\\
aes\_10\_1\_2\_4\_pp&  288 &  318  &
 0.22\secunit & 55.59\MBunit &
 0.44\secunit & 7.28\MBunit
\\
\hline
 mult3x3 &33 & 28 &
 0.01\secunit & 54.52\MBunit &
 0.00\secunit & 1.96\MBunit \\
 mult4x4 &55 & 48 &
 0.00\secunit & 54.54\MBunit &
 0.00\secunit & 1.95\MBunit \\
 mult5x5 & 83 & 74 &
 0.01\secunit & 54.66\MBunit &
 0.01\secunit & 1.95\MBunit \\
 mult6x6 & 117 & 106 &
 0.03\secunit & 54.92\MBunit &
 0.03\secunit & 1.95\MBunit \\
 mult8x8 & 203 & 188 &
 0.40\secunit & 55.43\MBunit &
 0.96\secunit & 2.21\MBunit \\
 mult10x10 & 313 & 294 &
 18.11\secunit & 85.91\MBunit &
 22.85\secunit & 3.61\MBunit 

\\
aes\_1\_2\_2\_4&  72 &  72  &
 3.53\secunit & 54.92\MBunit &
 0.08\secunit & 2.51\MBunit
\\
aes\_3\_1\_2\_4&  104 &  104  &
 0.48\secunit & 55.42\MBunit &
 0.23\secunit & 2.98\MBunit
\\
aes\_4\_1\_1\_4&  68 &  68  &
 0.14\secunit & 54.94\MBunit &
 0.01\secunit & 2.38\MBunit
\\
aes\_4\_1\_2\_4&  120 &  120  &
 0.88\secunit & 55.44\MBunit &
 0.32\secunit & 3.27\MBunit
\\
aes\_4\_2\_1\_4&  136 &  136  &
 0.63\secunit & 55.68\MBunit &
 1.36\secunit & 3.91\MBunit
\\
aes\_5\_1\_2\_4&  148 &  148  &
 1.29\secunit & 55.69\MBunit &
 0.40\secunit & 3.58\MBunit
\\
aes\_6\_1\_1\_4&  100 &  100  &
 0.17\secunit & 55.42\MBunit &
 0.04\secunit & 2.73\MBunit
\\
aes\_6\_1\_2\_4&  176 &  176  &
 1.55\secunit & 55.98\MBunit &
 0.64\secunit & 4.05\MBunit
\\
aes\_7\_1\_2\_4&  204 &  204  &
 1.62\secunit & 56.45\MBunit &
 0.37\secunit & 5.15\MBunit
\\
aes\_10\_1\_1\_4&  164 &  164  &
 0.26\secunit & 55.95\MBunit &
 0.02\secunit & 3.48\MBunit
\\
aes\_10\_1\_2\_4&  288 &  288  &
 2.93\secunit & 61.32\MBunit &
 0.43\secunit & 7.27\MBunit
\end{tabular}
}
\end{center}
\caption{Comparison of \PolyBoRi and MiniSat}
\label{tab:pb_sat}
\end{table}
%
Although, the memory consumption of \PolyBoRi is larger, \tabref{tab:pb_sat}
illustrates,
the computation time of both approaches is comparable for this kind of practical
examples. (Again the first part was computed using preprocessing.)
%
In  particular, it shows, that in our research area the algebraic
approach is competitive with SAT-solvers.

The advantages of \PolyBoRi were illustrated by the examples above as follows:
the fast Boolean multiplication can be seen in the
pigeon hole benchmarks.
%
The good performance of the cryptography examples is due to fast elimination of
auxiliary variables. The computations of the uuf problems include a large number
of generators, consisting of initially short polynomials, which 
lead to large intermediate results.
The algorithmic improvement of \symmgbGFTwo and the \optimised pair handling
render the treatment of these example with algebraic methods possible.

%* bessere resourcen als f4 (siehe magma manual)

In this way the initial performance of \PolyBoRi seems to be very promising. The
data shows, that the advantage of \PolyBoRi grows with the number of
variables. For many practical applications this size will be even bigger. We are
very confident, that it will be possible to tackle some of these problems in
future by using more \specialised approaches. This is a key point in the
development of \PolyBoRi to facilitate problem specific, high performance
solutions.


==> poly_as_set.tex <==
\section{Boolean Polynomials as Sets}
\label{sec:poly_as_set}

We are actually interested in \modelling expressions from propositional logic as
polynomials over the finite field with two elements. 
Allowing  values from~$\{0,1\}$ only, the condition~$x = x^2$ holds for
all~$x\in\Ztwo$.  
Hence, we deal with elements of the polynomial 
ring~$P = \Ztwoxoneton$ restricted by
the~\emph{field equations}
%
\begin{equation}
\label{eqn:fieldeqns}
x_1^2 = x_1,\, x_2^2 = x_2,\quad\cdots\quad,\, x_n^2 = x_n\mfstop
\end{equation}
%
This leads to a degree bound of one on all variables, and therefore 
we can restrict ourself to a certain class of polynomials in the
following. 
%
\begin{defn}[Boolean Polynomials]
\label{def:boolepoly}
Let~$p\in \Ztwoxoneton$ be a polynomial, \sth
%
\begin{equation}
\label{eqn:expandedpoly}
p =  a_1 \cdot x_1^{\nu_{11}} \cdot \ldots \cdot x_n^{\nu_{1n}}+ \ldots +
     a_m \cdot x_1^{\nu_{m1}} \cdot \ldots \cdot x_n^{\nu_{mn}}
\end{equation}
%
with coefficients~$a_i \in \{0, 1\}$ and~$\nu_{ij}\in\{0,1\}$.
Then~$p$ is called a \defemph{Boolean polynomial}.
%
%The set of all Boolean polynomials over~$\Ztwoxoneton$ is denoted by
%$\Bool_\Ztwoxoneton$, or just \Bool if there is now confusion about the polynomial
%ring.
\end{defn}
%
A given Boolean polynomial~$p$ is defined by the fact, whether 
each term~$x_1^{\nu_{i1}} \cdot \ldots \cdot x_n^{\nu_{in}}$ occurs in it.
Analogously, the occurrences of the variables determine each term. 
One can assign a set~$S_p= \{s_1, \,\cdots, s_m\}$ to~$p$ consisting of
different subsets~$s_k$,  $s_i \not= s_j$ for $i \not= j$, 
of the variable vector~$ \{x_1, \cdots, x_n\}$.
Then \eqnref{eqn:expandedpoly} can be rewritten as
%
\label{sec:rewrittenpoly}%
\begin{equation}
\label{eqn:rewrittenpoly}
p =  \sum_{s\in S_p} \left( \prod_{x_\nu \in s}x_\nu \right)
  \quad\mbox{with}\quad
S_p = \{ \underbrace{ \{x_{i_1}, \cdots,x_{i_{n_1}}\} }_{s_1}, \cdots, 
         \underbrace{ \{x_{i_m}, \cdots,x_{i_{n_m}}\} }_{s_m} \}
\mcomma
\end{equation}
%
with indices~$i_j\in\{1, \dots n\}$.
%
In fact, there is a  one-to-one correspondence
between the set of Boolean polynomials in~$P$ and the set of all subsets of the
power set of~$\{x_1, \dots, x_n\}$ via the mapping which is defined
by~$S_p \mapsto \sum_{s\in S_p} \left( \prod_{x_\nu \in s}x_\nu \right)=p$.


For practical applications it is reasonable to assume that~$S_p$ is sparse, \ie
the set is only a small subset of the power set over the variable
vector. Even the $s_i$ can be considered to be sparse, as usually 
quite few variables occur in a term.
Consequently, the strategies of the used algorithms have to be tuned in
such a way, that this kind of sparsity is preserved.

In our context it is enough to treat Boolean polynomials only, as
they are exactly the canonical representative of residue classes
in the quotient ring of~$\Ztwoxoneton$ modulo the ideal of the field equations% 
~$\explfieldideal$.



\subsection{Zero-suppressed Binary Decision Diagrams}
\label{sec:bdd}

Binary decision diagrams (BDDs) are widely used in various areas 
as a unique representation of large sets, which could not be
constructed efficiently by an enumerative approach.

\begin{defn}[Binary Decision Diagram]

A \defemph{binary decision diagram}~(BDD) is a rooted, directed, and acyclic
graph with two terminal nodes~$\{0, 1\}$ and decision nodes.
The latter have two ascending edges~(high/low or then/else),
each of which corresponding to the assignment of true or false, respectively, to
a given Boolean variable.

A series of connected nodes of a BDD starting at the root and ending at the
terminal node~1 is called a~\defemph{path}.
%
In case, that the variable order is constant over all
paths, we speak of an \defemph{ordered} BDD.

\end{defn}

This data structure is compact and easy to handle.
%
For a more detailed treatment of the subject 
see~\cite{Bryant86} and~\cite{berardetal01}.


\begin{defn}
Let~$b$ be a binary decision diagram.
\begin{itemize}
\item
The decision variable associated to the root node of~$b$ is denoted
by~$\mathrm{top}(b)$. Furthermore,
$\thenBranch(b)$ and~$\elseBranch(b)$ indicate
the (sub-)diagrams, linked to then- and else-edge, respectively, of the root
node of~$b$.
\item For two BDDs~$b_1, b_0$, which do not depend on the
decision variable~$x$, the \defemph{if-then-else operator}
$ite(x,b_1,b_0)$ denotes the BDD~$c$, which is obtained by introducing
a new node associated to the variable~$x$, \sth~$\thenBranch(c) = b_1$,
and~$\elseBranch(c) = b_0$.
\end{itemize}
\end{defn}

The set of all valid paths of a binary decision diagrams can be used to
represent a subset of the power set of the decision variables, 
which can be accessed easily, by following then- and else-edges.
Since  any Boolean polynomial~$p$ can be identified uniquely with such 
subset, BDDs are perfectely  suited  for storing Boolean polynomials in a
natural way.  
For instance, \figref{fig:zdd_motiv} shows some BDDs for~$p=a\,c +c$.
%
\begin{figure}
\begin{center}
\subfigure[non-canonical]{%
\phantom{(b)~}\hspace{1.5em}%
\includegraphics[scale=0.225]{zdd_motiv_2}\label{fig:zdd_motiv_2}
\hspace{1.5em}
}%
\subfigure[zero-supressed]{%
\phantom{(c)~}\hspace{1.5em}%
\includegraphics[scale=0.225]{zdd_motiv_3}\label{fig:zdd_motiv_3}
\hspace{1.5em}%
}%
\end{center}
\caption{Different binary decision diagrams representing~$a\, c+c$.
Edges:~$\thenBranch$~(---) and $\elseBranch$~(- -).
\label{fig:zdd_motiv}}
\end{figure}%
%
Unlike other BDD approaches, the diagram paths do not represent
the valid solutions of the Boolean function behind~$p$, but they form the
sets~$\{a, c\}$ and~$\{c\}$ corresponding to polynomial terms directly.

For efficiency reasons it is useful to omit variables, which are not necessary
to construct the whole set. A classic variant for this purpose is the
\defemph{reduced-ordered BDD}~(ROBDD, sometimes referred to as ``\emph{the}
BDD''). These are ordered BDDs with equal subdiagrams merged,
\ie if some edges point to equivalent subdiagrams, those are forced to point to
the same diagram and share it. Furthermore, a node elimination is applied, if
both descending edges point to the same node.

While the last reduction rule is useful for describing numerous Boolean-valued
vectors, it is gainless for treating sparse sets. For this case,
another variant, namely the ZDD~(sometimes also called~ZBDD or~ZOBDD),
has been introduced.

\begin{defn}[ZDD]
Let~$z$ be an ordered binary decision diagram with equal subdiagrams merged.
Then~$z$ is called a \defemph{zero-suppressed binary decision
diagram}~(ZDD), if and only if those nodes are eliminated, whose then-edges
point to 
the~$0$-terminal.
\end{defn}

Note, in this case elimination means, that a nodes~$n$ is removed from the
diagram and all edges pointing to it are linked to~$\elseBranch(n)$.
%
\Figref{fig:zdd_motiv} illustrates this reduction step of a given 
binary decision diagram  for the
polynomial~$a\,c +c$.
%
In \figref{fig:zdd_motiv_2} the then-edge of the right node with decision
variable~$c$  is pointing to the 0-terminal. Hence, it can be safely removed,
without losing information.
As a consequence, the then-edge of the $b$-node is now connected to zero, and hence can
also be eliminated.
The effect of the complete zero-suppressed node reduction can be seen in
\figref{fig:zdd_motiv_3}.
%
Note, that the construction guarantees canonicity of resulting
diagrams, see~\cite{Ghasemzadeh05}.
%
But still the structure of resulting decision diagrams depends on the order of
variables. 
%
\Figref{fig:zdd_expl} shows
example ZDDs for a given Boolean polynomial.
%
\begin{figure}[htb!]
\begin{center}
\subfigure[$a,b,c$]{%
\includegraphics[scale=0.25]{zdd_abc.pdf}\label{fig:zdd_abc}
}% 
\subfigure[$a,c,b$]{%
\hspace{1.5em}%
\includegraphics[scale=0.25]{zdd_acb.pdf}\label{fig:zdd_acb}
}%
\end{center}
\caption{ZDDs representing the polynomial~$a\,c+b\,c+c$ for 
two different variable orders.
Edges:~$\thenBranch$~(---) and $\elseBranch$~(- -).
\label{fig:zdd_expl}}
\end{figure}%
%
In particular, the number of diagram nodes is highly sensitive to
it, as \figname{}s~\ref{fig:zdd_abc} and~\ref{fig:zdd_acb} illustrate.
Therefore, a suitable choice of the order is always a crucial point,
when \modell{}ing a problem using sets of Boolean polynomials.



==> post_intro.tex <==
Following, we start with a motivation of suitable data structures for handling
of Boolean polynomials and continue with some mathematical background.
Then we give a brief description of the \PolyBoRi framework and the implemented
algorithms. Finally, the treatment of some benchmark examples is compared with
those of other computer algebra systems.


==> problem.tex <==
\section{Introduction}
\Groebner bases have become a standard tool for treating
problems which can be described by polynomial systems.
%
While the concept of \Groebner bases is known much longer, their current 
practical importance is a result of dramatical improvements in performance and 
algorithms in recent years.
%
It has also been shown, that a \specialised implementation can often tackle much
harder problems, like \citeauthor{Fau:03}'s  HFE-attacks \citeyearpar{Fau:03}.
%(\eg Allan Steels HFE-attacks in \Magma).
The motivation for our work was to provide a framework for computations
in the following special but nevertheless important case of polynomials: 
coefficients lie in the field
with two elements and exponents are bounded to degree one in each variable. This
degree bound usually originates from the application of field equations of the
form $x^2=x$. This occurs in many significant applications 
like formal verification, but also in cryptography, logic, and many more. This is
due to the fact that those special polynomials~-- the so-called Boolean
polynomials~-- correspond directly to Boolean
functions.

Although the treatment of polynomial systems using \Groebner bases 
improved considerably in recent years, current implementations have not been
capable of 
satisfactorily handling Boolean polynomials from real-world applications yet.
%
One of the first questions was: Can we use the properties of this simplified
class of polynomials to obtain better data structures?
Of course, we did also ask, whether we can find  algorithmic improvements in
this situation.



The role of \PolyBoRi in this context is to provide a framework of high performance data structures and example \Groebner bases algorithms.
On the other hand  it is very clear, that many problems arising from 
% Rem: as noun usually ``practice'' also in BE
practice can only be tackled, if \optimis{}ation occurs on many levels: 
data structures, higher level algorithms, formulation of equations/problems, good monomial orderings\ldots

An important aspect in symbolic computation is that~-- independent of the
strategy~-- 
polynomials can become very big, but usually keep structured (in a very general
sense). Using this structure to keep the memory consumption moderate was a
primary design goal of \PolyBoRi.  Another observation is that
operations on similar polynomials (differing
only in a few terms) occur quite often during \Groebner basis
computations. \PolyBoRi also gives an answer to that problem using
a cache mechanism on the level of polynomial substructures.



==> results.tex <==
%\addvspace{2ex}% some space to force table below completely on next page
\section{Benchmarks and Practical Results}
\providecommand{\secunit}{\ensuremath{\,\mathrm{s}}}
\providecommand{\MBunit}{\ensuremath{\,\mathrm{MB}}}

\providecommand{\timedoutAfter}[1]{\multicolumn{1}{c}{$\infty$} & }
\providecommand{\memoryout}{ &\,\hfill$\infty$\hfill\, }
% Alternative, explicitely stating time/memory excess
\renewcommand{\timedoutAfter}[1]{\multicolumn{1}{c}{\!\!$>$#1\!\!}&}
\renewcommand{\memoryout}{&\!\!\!\,\hfill$>\!\!15\,\mathrm{GB}$\hfill\,\!\!\! }
\providecommand{\timedout}{\timedoutAfter{1\,h}}


This section presents some benchmarks comparing \PolyBoRi to general purpose and \specialised computer algebra systems.
Note, that it only presents the state of \PolyBoRi in the development version at the end of August~2007. Since the project is very young we can expect major performance improvements for sure in the near future.

The following timings have been done on a AMD Dual Opteron 2.2 GHz (all systems have used only one CPU) with 16 GB RAM on Linux.

The used ordering was lexicographical, with the exception of FGb, where
degree-reverse-lexicographic was used. \PolyBoRi also implements degree ordering, but for the presented practical examples elimination orderings seem to be more appropriate. A recent development in \PolyBoRi was the implementation of block orderings, which behave very natural for many examples.


We compared the following system releases with the development version
of \PolyBoRi's \symmgbGFTwo:

\begin{tabular}{lll}
Maple& 11.01, June 2007 & Gr\"obner package, default options\\
FGb &  1.34, Oct.\ 2006 &  via Maple 11.01, command: fgb\_gbasis\\
\Magma & 2.13-10, Feb.\ 2007&  command: GroebnerBasis, default options\\
\Singular& 3-0-3, May 2007 & std, option(redTail)\\% (= \PolyBoRi's default) 
\end{tabular}

% Note, that this  presents the state of
%\PolyBoRi in the development version  in August 2007 only. Since the
%project is still very young there is still room for major performance
%improvements.



The examples were chosen from current research problems in formal verification
and algebraic crypto analysis.
The latter yields systems of equations, which are comparable to those arising
from formal verification, but they are more scalable.
%
We use an algebraic attack to a small scale variant of the
\emph{Advanced Encryption Standard}~(AES)~\citep{FIPS197}.
This approach is based on~\cite{CidMurRob05} and
was provided by Stanislav Bulygin~\citetext{private communication}.  We made
some \optimisations on the
formulation of the equations in the formulation.
This is done by an approach similar to the one of \cite{ToliZ04}, but
over~GF2.
Details will be published in a later article. 

Furthermore,  examples using \emph{Courtois Toy Cipher}~(CTC),
which are due to Martin Albrecht~\citep{AlbrechtM}, were tested.
The systems describing the formal verification of
multipliers were provided by Markus Wedler~\citetext{private communication}.


All timings of the computations are \summarised in \tabref{table:results} below.
%
% Status: 2007-08-20, 2007-08-28 (fgb + PolyBoRi memory peak)
\begin{table}
\begin{center}
{\tiny
\newcommand{\cstyle}{{\hspace{.6em}}}
\renewcommand{\MBunit}{}
\renewcommand{\secunit}{}
\begin{tabular}{crr|rr||@{\cstyle}r@{\cstyle}r@{\cstyle}|@{\cstyle}r@{\cstyle}r@{\cstyle}|@{\cstyle}r@{\cstyle}r@{\cstyle}|@{\cstyle}r@{\cstyle}r@{\cstyle}}
\multicolumn{3}{c}{} & \multicolumn{2}{c}{\PolyBoRi} & 
  \multicolumn{2}{c}{FGb}&
  \multicolumn{2}{c}{Maple}&
  \multicolumn{2}{c}{\Magma} & \multicolumn{2}{c}{\Singular}
\\
Example &\multicolumn{2}{@{\cstyle}c|}{Vars./Eqs.} &

\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c||@{\cstyle}}{MB} &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c|@{\cstyle}}{MB} &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c|@{\cstyle}}{MB} &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c|@{\cstyle}}{MB}  &
\multicolumn{1}{@{\cstyle}c}{s} & \multicolumn{1}{@{\cstyle}c}{MB}

\\
\hline
aes\_7\_1\_2\_4\_pp&  204 &  225  &
0.15\secunit & 53.82\MBunit
& % Format: fgb
2812.30\secunit & 10.12\MBunit
 & %Format : maple
\timedout %0.70\secunit &  11.00\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
346.37\secunit & 206.22\MBunit
 & %Format : sing
27.41\secunit & 25.77\MBunit
\\
aes\_10\_1\_1\_4\_pp&  164 &  184  &
0.02\secunit & 52.70\MBunit
& % Format: fgb
1.97\secunit & 9.37\MBunit
 & %Format : maple
2.99\secunit & 10.37\MBunit
 & %Format : magma
0.87\secunit & 9.03\MBunit
 & %Format : sing
0.02\secunit& 1.75\MBunit
\\
aes\_10\_1\_2\_4\_pp&  288 &  318  &
0.22\secunit & 55.59\MBunit
& % Format: fgb
\timedout %Error:1.960\secunit & 10.37\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %1.36\secunit & 12.50\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
847.91\secunit & 471.58\MBunit
 & %Format : sing
183.73\secunit & 55.86\MBunit
\\


ctc\_3\_3&  117 &  117  &
0.04\secunit & 52.80\MBunit
& % Format: fgb
6.56\secunit & 8.62\MBunit
 & %Format : maple
10.40\secunit &  10.37\MBunit
 & %Format : magma
1.62\secunit & 10.39\MBunit
 & %Format : sing
0.77\secunit & 5.25\MBunit
\\
ctc\_5\_3&  189 &  189  &
0.10\secunit & 63.05\MBunit
& % Format: fgb
602.20\secunit & 9.75\MBunit
 & %Format : maple
929.77\secunit & 10.87\MBunit
 & %Format : magma
85.20\secunit & 67.79\MBunit
 & %Format : sing
3.63\secunit & 14.75\MBunit
\\
ctc\_8\_3&  297 &  297  &
0.15\secunit & 64.23\MBunit
& % Format: fgb
\timedout%Error:0.920\secunit & 9.87\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %0.86\secunit & 12.50\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
759.51\secunit & 299.08\MBunit
 & %Format : sing
14.32\secunit & 33.31\MBunit
% End of sing
\\
ctc\_15\_3&  549 &  549  &
0.28\secunit & 68.71\MBunit
& % Format: fgb
\timedout%Error:3.020\secunit & 11.25\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %2.67\secunit &  17.12\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
\timedout
 & %Format : sing
66.63\secunit & 116.98\MBunit
\\
\hline
mult3x3&  33 &  28  &
0.01\secunit & 54.52\MBunit
& % Format: fgb
0.07\secunit & 3.50\MBunit
 & %Format : maple
0.04\secunit & 3.00\MBunit
 & %Format : magma
0.57\secunit & 6.55\MBunit
 & %Format : sing
0.01\secunit & 0.64\MBunit
\\
mult4x4&  55 &  48  &

 0.00\secunit & 54.54\MBunit
& % Format: fgb
1.76\secunit & 5.50\MBunit
 & %Format : maple
1.96\secunit & 4.87\MBunit
 & %Format : magma
0.91\secunit & 10.48\MBunit
 & %Format : sing
0.02\secunit & 0.66\MBunit
\\
mult5x5&  83 &  74  &

 0.01\secunit & 54.66\MBunit
& % Format: fgb
219.09\secunit & 6.37\MBunit
 & %Format : maple
236.14\secunit &  6.87\MBunit
 & %Format : magma
31.28\secunit & 46.05\MBunit
 & %Format : sing
0.01\secunit & 1.67\MBunit
\\
mult6x6&  117 &  106  &
0.03\secunit & 54.92\MBunit
& % Format: fgb
\multicolumn{2}{c|@{\cstyle}}{failed}%
%bytes used=17585984, alloc=9304408, time=0.28
%Error, (in FGb:-fgb_gbasis) Limite de to_do est a 348406 !
 & %Format : maple
\timedout %3586.97\secunit & 1148.16\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
\timedout
 & %Format : sing
4.28\secunit & 21.19\MBunit
\\
mult8x8&  203 &  188  &

0.40\secunit & 55.43\MBunit
& % Format: fgb
\timedout%Error:3.210\secunit & 63.36\MBunit
% fatal error, lost connection to kernel
 & %Format : maple
\timedout %2.93\secunit & 50.99\MBunit
% fatal error, lost connection to kernel
 & %Format : magma
\timedout
 & %Format : sing
\memoryout   %2.17\secunit & error: no more memory bytes
\\
mult10x10&  313 &  294  &

 18.11\secunit & 85.91\MBunit
& % Format: fgb
\memoryout
 & %Format : maple
\memoryout & %Execution Stopped: Memory allocation failed
 %Format : magma
\memoryout & %Format : sing
\memoryout %220.37\secunit & error: no more memory bytes
\end{tabular}
}
\end{center}
\caption{Timings and memory usage for benchmark examples.}
\label{table:results}
\end{table}
%
The authors of this article are quite convinced, that the default strategy of
\Magma\ is not well suited for these examples (walk, see \citet{CoKaMa97}, or \homogenisation). However, when we tried a direct approach in \Magma, it ran very fast out of memory~(at least in the larger examples). So we can conclude, that the implemented \Groebner basis algorithm in \PolyBoRi offers a good performance combined with low memory consumption.
The relatively large offset of about~$50\,\mathrm{MB}$ in  memory
usage  is due to an initial memory pool for the cache 
management, whose size depends on the available RAM.
Part of the strength in directly computing \Groebner bases (without walk or similar techniques) is inherited from the slimgb algorithm in \Singular.
On the other hand our data structures provided a fast way to rewrite polynomials, which might be of bigger importance than sparse strategies in the presented examples.
%
While we used the normal slimgb algorithm for the presented examples, we were able to tackle much harder problems like~12-BIT-Multiplier, AES small scale chiffre SR(10-1-2-8), SR(10-2-1-8),  SR(10-2-2-4) using \optimis{}ed scripts.


In order to treat classes of examples, for which the lexicographical ordering is
not the best choice, \PolyBoRi is also equipped with other monomial orderings. 
Although, its internal data structure is ordered lexicographically, 
the computational overhead of the degree orderings implementation is small
enough, that the advantage of these orderings become effect.
%
\Tabref{tab:orderbench} illustrates this for a series of random unsatisfiable
examples~\cite{satlib00}. The latter arise from benchmarking SAT-solvers, which can handle them
very quickly, as their conditions are easy to contradict. But they are still a
challenge for the algebraic approach.
%
\begin{table}
\begin{center}
{\tiny
\begin{tabular}{@{}cccc|rr||rr|rr@{}}
 % \multicolumn{4}{c}{} & 
 % \multicolumn{2}{c}{\PolyBoRi} &
 % \multicolumn{2}{c}{\Magma} & 
 % \multicolumn{2}{c}{FGb} 
\\
Example &\multicolumn{2}{c}{Vars./Eqs.} & Order. &

  \multicolumn{2}{c||}{\PolyBoRi} &
  \multicolumn{2}{c|}{\Magma} & 
  \multicolumn{2}{c}{FGb} 

%\multicolumn{1}{c}{s} & \multicolumn{1}{c||}{MB} &
%\multicolumn{1}{c}{s} & \multicolumn{1}{c|}{MB}  &
%\multicolumn{1}{c}{s} & \multicolumn{1}{c}{MB} 
\\
\hline
uuf50\_8&  50 &  218  &
lp &
11.58\secunit & 71.58\MBunit
 & %Format : magma
12.88\secunit & 26.04\MBunit
   \\
&&& dlex&
10.95\secunit & 71.06\MBunit
 & %Format : magma
13.45\secunit & 29.02\MBunit
   \\
&&&dp\_asc&
7.78\secunit & 70.82\MBunit
 & %Format : magma
9.83\secunit & 37.02\MBunit
 & %Format : FGb
76.27\secunit & 6.75\MBunit
\\
\begin{comment}
%lp
uuf50\_9&  50 &  218  &
lp&
8.48\secunit & 71.12\MBunit
 & %Format : magma
14.82\secunit & 34.68\MBunit
   \\
&&&dlex&
10.15\secunit & 71.36\MBunit
 & %Format : magma
13.37\secunit & 36.45\MBunit
    \\
&&&dp\_asc &
14.11\secunit & 74.77\MBunit
 & %Format : magma
13.12\secunit & 33.06\MBunit
 & %Format : FGb
92.53\secunit & 6.75\MBunit
\\
uuf50\_10&  50 &  218  &
lp &
8.76\secunit & 71.98\MBunit
 & %Format : magma
9.77\secunit & 28.21\MBunit
   \\
&&& dlex&
8.98\secunit & 72.53\MBunit
 & %Format : magma
10.35\secunit & 32.71\MBunit
   \\
 &&& dp\_asc&
8.14\secunit & 72.24\MBunit
 & %Format : magma
8.40\secunit & 27.42\MBunit
 & %Format : GFb
74.76\secunit & 6.75\MBunit
\\
\end{comment}
uuf75\_8&  75 &  325  &
lp &
843.38\secunit & 819.80\MBunit
 & %Format : magma
14015.21\secunit & \!\!\!\!\!1633.62\MBunit
   \\
&&& dlex &
553.43\secunit & 490.86\MBunit 
 & %Format : magma
14291.45\secunit & \!\!\!\!\!2439.53\MBunit
   \\
 &&& dp\_asc&
448.53\secunit & 472.04\MBunit 
 &  %Format : magma
13679.42\secunit &\!\!\!\!\! 2539.24\MBunit
& % Format: FGb
\!\!\!99721.46\secunit    & \!\!\!\!\!\!8958.36\MBunit% \timedoutAfter{24\,h}
\\
uuf100\_01&  100 &  430  &
lp &
44779.77\secunit & \!\!\!\!\!12309.79\MBunit
 & %Format : magma
 \timedoutAfter{2\,days}
\\
  &&&dlex &
11961.86\secunit & 6101.43\MBunit
& %Format : magma
 \timedoutAfter{2\,days}
\\
&&&dp\_asc &
10635.72\secunit & 6146.47\MBunit 
 & %Format : magma
\timedoutAfter{2\,days} 
& % Format: FGb
\multicolumn{2}{c}{failed}
% at sculptor, 2.4GHz alloc=9959648, time=57135.11
%Error, (in FGb:-fgb_gbasis) Limit for allocations (1-->1000): in
%update_all_garbages !
\end{tabular}
}
\end{center}

\caption{Timings and memory usage for benchmark examples, w.\,r.\,t.\ various
orderings. 
%The infinity symbols mark timeout after two days.
%The infinity symbols in time and memory columns
%mark timeout after one day and out of memory, respectively.
}
\label{tab:orderbench}
\end{table}
%
The strength of \PolyBoRi is visible in the more complex examples, as it scales
better than the other systems in tests.
% REM: uuf erst mal draussen? - Wieder drin, zur Illustraiion deg-order
The computations of the these problems include a large number
of generators, consisting of initially short polynomials, which 
lead to large intermediate results.
The algorithmic improvement of \symmgbGFTwo and the \optimised pair handling
render the treatment of these example with algebraic methods possible.

In addition the performance of \PolyBoRi is compared  with the freely
available SAT-solver MiniSat2~(release date 2007-07-21),  which is
state-of-the-art
among publicly available solvers~\citep{een03minisat}.
The examples consist of formal verification
examples corresponding to digital circuits with $n$-bitted multipliers
and the pigeon hole benchmark, which is the most important
standard benchmark problem for
SAT-solvers, \eg used in in~\cite{satlib00}, and some small-scale AES examples
again.
The latter checks whether it is possible to place~$n+1$ pigeons in~$n$ holes
without two of them being in the same hole~(obviously, it is unsatisfiable).

%minisat2 2007-07-21
%
\begin{table}[bth]
\begin{center}
{\tiny
\begin{tabular}{l|rr|rr|rr}
& \multicolumn{2}{c|}{Vars./Eqs.}  &
    \multicolumn{2}{c|}{\PolyBoRi}  &  \multicolumn{2}{c}{MiniSat}  \\
\hline
 hole6 & 42 & 133 &
 0.13\secunit & 51.64\MBunit &
 0.01\secunit & 1.96\MBunit \\
 hole7 & 56 & 204 &
 0.46\secunit & 51.89\MBunit &
 0.06\secunit & 1.96\MBunit \\
 hole8 & 72 & 297 &
 1.88\secunit &56.59\MBunit &
 0.30\secunit & 2.08\MBunit \\
 hole9 & 90 & 415 &
 8.01\secunit & 84.04\MBunit &
 2.31\secunit & 2.35\MBunit \\
 hole10 & 110 & 561 &
 44.40\secunit & 97.68\MBunit &
 25.20\secunit & 3.24\MBunit \\
aes\_2\_2\_2\_4&  128 &  128  &
 3.93\secunit & 64.91\MBunit &
 12.04\secunit & 4.73\MBunit
\\
aes\_3\_2\_2\_4&  184 &  184  &
 46.67\secunit & 88.77\MBunit &
 76.88\secunit & 6.77\MBunit
\\
aes\_10\_1\_1\_8&  328 &  328  &
 2.26\secunit & 132.74\MBunit &
 58.30\secunit & 38.13\MBunit
\\
aes\_10\_2\_2\_4&  576 &  576  &
 1193.19\secunit & 150.70\MBunit &
 190.58\secunit & 15.03\MBunit
\\
aes\_7\_1\_2\_4\_pp&  204 &  225  &
 0.15\secunit & 53.82\MBunit &
 0.38\secunit & 5.16\MBunit
\\
aes\_10\_1\_1\_4\_pp&  164 &  184  &
 0.02\secunit & 52.70\MBunit &
 0.03\secunit & 3.49\MBunit
\\
aes\_10\_1\_2\_4\_pp&  288 &  318  &
 0.22\secunit & 55.59\MBunit &
 0.44\secunit & 7.28\MBunit
\\
\hline
 mult3x3 &33 & 28 &
 0.01\secunit & 54.52\MBunit &
 0.00\secunit & 1.96\MBunit \\
 mult4x4 &55 & 48 &
 0.00\secunit & 54.54\MBunit &
 0.00\secunit & 1.95\MBunit \\
 mult5x5 & 83 & 74 &
 0.01\secunit & 54.66\MBunit &
 0.01\secunit & 1.95\MBunit \\
 mult6x6 & 117 & 106 &
 0.03\secunit & 54.92\MBunit &
 0.03\secunit & 1.95\MBunit \\
 mult8x8 & 203 & 188 &
 0.40\secunit & 55.43\MBunit &
 0.96\secunit & 2.21\MBunit \\
 mult10x10 & 313 & 294 &
 18.11\secunit & 85.91\MBunit &
 22.85\secunit & 3.61\MBunit 

\\
aes\_1\_2\_2\_4&  72 &  72  &
 3.53\secunit & 54.92\MBunit &
 0.08\secunit & 2.51\MBunit
\\
aes\_3\_1\_2\_4&  104 &  104  &
 0.48\secunit & 55.42\MBunit &
 0.23\secunit & 2.98\MBunit
\\
aes\_4\_1\_1\_4&  68 &  68  &
 0.14\secunit & 54.94\MBunit &
 0.01\secunit & 2.38\MBunit
\\
aes\_4\_1\_2\_4&  120 &  120  &
 0.88\secunit & 55.44\MBunit &
 0.32\secunit & 3.27\MBunit
\\
aes\_4\_2\_1\_4&  136 &  136  &
 0.63\secunit & 55.68\MBunit &
 1.36\secunit & 3.91\MBunit
\\
aes\_5\_1\_2\_4&  148 &  148  &
 1.29\secunit & 55.69\MBunit &
 0.40\secunit & 3.58\MBunit
\\
aes\_6\_1\_1\_4&  100 &  100  &
 0.17\secunit & 55.42\MBunit &
 0.04\secunit & 2.73\MBunit
\\
aes\_6\_1\_2\_4&  176 &  176  &
 1.55\secunit & 55.98\MBunit &
 0.64\secunit & 4.05\MBunit
\\
aes\_7\_1\_2\_4&  204 &  204  &
 1.62\secunit & 56.45\MBunit &
 0.37\secunit & 5.15\MBunit
\\
aes\_10\_1\_1\_4&  164 &  164  &
 0.26\secunit & 55.95\MBunit &
 0.02\secunit & 3.48\MBunit
\\
aes\_10\_1\_2\_4&  288 &  288  &
 2.93\secunit & 61.32\MBunit &
 0.43\secunit & 7.27\MBunit
\end{tabular}
}
\end{center}
\caption{Comparison of \PolyBoRi and MiniSat}
\label{tab:pb_sat}
\end{table}
%
Although, the memory consumption of \PolyBoRi is larger, \tabref{tab:pb_sat}
illustrates,
the computation time of both approaches is comparable for this kind of practical
examples. (Again the first part was computed using preprocessing.)
%
In  particular, it shows, that in our research area the algebraic
approach is competitive with SAT-solvers:
the fast Boolean multiplication can be seen in the
pigeon hole benchmarks.
%
In contrast, the good performance of the cryptography examples is due to fast
elimination of auxiliary variables. 



\section{Conclusions}
In this paper the \PolyBoRi framework was presented. It \utilises special
properties of Boolean systems of equations for computing \Groebner basis over
Boolean polynomials in an efficient way. A special data structure based on
binary decision diagrams, and \optimised procedures for polynomial operations
were  proposed. In addition, novel theoretical results were given, which have
been used to improve the algorithmic aspects in higher levels of the \Groebner
basis computations. 

On the one hand, \PolyBoRi offers fast Boolean operations and  elimination of
auxiliary variables. 
On the other, the algorithmic improvement of \symmgbGFTwo and the \optimised
pair handling make it possible to treat problems with a large number
of  generators, which might yield  large intermediate results.


It is also important to note, that various nontrivial monomial orderings were made
available in an efficient way on a ZDD-based data structure.
To our knowledge, this is a unique approach in area of \Groebner basis
computations, which already payed off. Also, together with some valueable
properties of binary decision diagrams it may lead to interesting new points of
view in future research. 

In this way the initial performance of \PolyBoRi seems to be very promising. It
can be seen, that the advantage of \PolyBoRi grows with the number of
variables. 
%
For many practical applications this size will even be bigger. We are very
confident, that it will be possible to tackle some of these problems in future
by using more \specialised approaches. Indeed, it was a key point during  the development of \PolyBoRi to facilitate problem specific, high performance solutions.


==> state_of_art.tex <==
\subsection{State of the Art}
\label{sec:state_of_art}

Although graph-based approaches using decision diagrams for polynomials were
already proposed before, those were not capable of handling
algebraic problems efficiently.
This was mainly due to the fact that the attempts were applied
to very general polynomials, which cannot be represented as binary
decision diagrams in a natural way.
% The latter leads to an computational overhead. 

For instance, the use of ZDDs for representing polynomials
with integer coefficients can be found in \cite{Minato95}.
In this context coefficients and degrees had to be coded in a binary manner,
which had lead to large diagram trees, even for rather small polynomials. 
Assuming bit length of~$m$ for each polynomial variable~$x_\nu$, a number 
of~$m$
decision variables has to be introduced in order to represent~$x_\nu^1,
x_\nu^2, \cdots, x_\nu^{2^m}$. 
Arbitrary~$x_\nu^n$ may be obtained by decomposing~$n$ into a sum of exponentials
with respect to base~$2$. The same can be done to binary encode the
coefficients. For instance, the polynomial~$5\,x^2+2\,x\,y$ has to be decomposed
into~$x^2 + 2^2\,x^2+2^1\,x^1\,y^1$, with the new set of
decision ``variables''~$\{x^2,x^1,y^1, 2^2, 2^1\}$. 

In this general case addition and multiplication correspond to costly set
operations involving de- and recoding of coefficient and degree
numbers. Another reason, why ZDDs were not used in computer algebra before, is
the importance of nontrivial monomial orderings. Usually, computer algebra
systems store polynomials with respect to the current monomial ordering \citep{BS:98}. This
enables fast access to the leading term, and efficient iterations over all
terms. In contrast, binary decision diagrams are ordered naturally in a
lexicographical way. Fortunately, for special cases like the Boolean polynomials
described in \secref{sec:poly_as_set}, it is possible to implement a search for
the leading term and term iterators with suitable effort. Also, the special case of
Boolean polynomials can be mapped to ZDDs more naturally, since the polynomial variables
are in one-to-one correspondence with the decision variables in the diagram. The
same applies for the polynomial arithmetic, which can efficiently be done using
basic set operations.  The \PolyBoRi framework presented in this work is addressed to the
\utilisation of this in a user-friendly environment.

Our approach can also be considered in the context of the meta approach
of~\cite{coudert92implicit}.  Boolean variables~$x_1, \cdots, x_n$ yield~$2^n$
possible configurations in~$\{0, 1\}^n$ for assigning true or false to
each~$x_\nu$. Enumerating all valid solution vectors with respect to rather simple
relations leads quickly to large and dense subsets of~$\{0, 1\}^n$. Since those
sets cannot be handled efficiently, it had been suggested to store and
manipulate the relations, which implicitly define the sets.
%
In the language of computer algebra, the implicit relations are systems of
Boolean polynomials. Hence, we can draw profit from the experience with
Gr{\"o}bner bases computations and heuristics for the treatment of polynomial
systems. In addition, especially tuned strategies can be refined and developed when
obeying the unique properties of Boolean rings.

